From globular clusters to the disc: the dual life of our Galaxy

The halo and disc globular cluster population can be used as a tracer of the primordial epochs of the Milky Way formation. In this work, literature data of globular clusters ages, chemical abundances, and structural parameters are studied, explicitly focussing on the origin of the known split in the age-metallicity relation of globular clusters. When the alpha-element abundances, which are less strongly affected by the internal light-element spread of globular clusters (Si, Ca), are considered, a very low observational scatter among metal-poor clusters is observed. A plateau at [SiCa/Fe]~0.35 dex, with a dispersion of only 0.05 dex is observed up to a metallicity of about -0.75 dex. Only a few metal-poor clusters in this metallicity interval present low [SiCa/Fe] abundances. Moreover, metal-rich globular clusters show a knee in the [alpha/Fe] versus [Fe/H] plane around [Fe/H] -0.75 dex. As a consequence, if a substantial fraction of galactic globular clusters has an external origin, they have to be mainly formed either in galaxies that are massive enough to ensure high levels of [alpha/Fe] element abundances even at intermediate metallicity, or in lower mass dwarf galaxies accreted by the Milky Way in their early phases of formation. Finally, clusters in the metal-poor branch of the AMR present an anti-correlation of [SiCa/Fe] with the total cluster magnitude, while this is not the case for metal-rich branch clusters. In addition, this lack of faint high-alpha clusters in the young metal-poor population is in contrast with what is observed for old and more metal-poor clusters, possibly reflecting a higher heterogeneity of formation environments at lower metallicity. Accretion of high-mass satellites, as a major contribution to the current Milky Way globular cluster system both in the metal-poor and the metal-intermediate regime is compatible with the observations.

==> biblio <==
@ARTICLE{MyeongSausage,
   author = {{Myeong}, G.~C. and {Evans}, N.~W. and {Belokurov}, V. and {Sanders}, J.~L. and 
	{Koposov}, S.~E.},
    title = "{The Sausage Globular Clusters}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1805.00453},
 keywords = {galaxies: kinematics and dynamics, galaxies: structure },
     year = 2018,
    month = aug,
   volume = 863,
      eid = {L28},
    pages = {L28},
      doi = {10.3847/2041-8213/aad7f7},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2018ApJ...863L..28M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kruijssen18,
   author = {{Kruijssen}, J.~M.~D. and {Pfeffer}, J.~L. and {Reina-Campos}, M. and 
	{Crain}, R.~A. and {Bastian}, N.},
    title = "{The formation and assembly history of the Milky Way revealed by its globular cluster population}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1806.05680},
 keywords = {Galaxy: evolution, Galaxy: formation, (Galaxy:) globular clusters: general, Galaxy: halo, Galaxy: stellar content, galaxies: star formation},
     year = 2018,
    month = jun,
      doi = {10.1093/mnras/sty1609},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.tmp.1537K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{AminaEnceladus,
   author = {{Helmi}, A. and {Babusiaux}, C. and {Koppelman}, H.~H. and {Massari}, D. and 
	{Veljanoski}, J. and {Brown}, A.~G.~A.},
    title = "{The formation of two of the major structural components of the Milky Way}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1806.06038},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2018,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2018arXiv180606038H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harris14,
   author = {{Harris}, W.~E. and {Morningstar}, W. and {Gnedin}, O.~Y. and 
	{O'Halloran}, H. and {Blakeslee}, J.~P. and {Whitmore}, B.~C. and 
	{C{\^o}t{\'e}}, P. and {Geisler}, D. and {Peng}, E.~W. and {Bailin}, J. and 
	{Rothberg}, B. and {Cockcroft}, R. and {Barber DeGraaff}, R.
	},
    title = "{Globular Cluster Systems in Brightest Cluster Galaxies: A Near-universal Luminosity Function?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1410.6291},
 keywords = {galaxies: formation, galaxies: star clusters: general, globular clusters: general},
     year = 2014,
    month = dec,
   volume = 797,
      eid = {128},
    pages = {128},
      doi = {10.1088/0004-637X/797/2/128},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014ApJ...797..128H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Eu10PCA,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R.~G. and 
	{Recio-Blanco}, A. and {Lucatello}, S. and {D'Orazi}, V. and 
	{Cassisi}, S.},
    title = "{Properties of stellar generations in globular clusters and relations with global parameters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1003.1723},
 keywords = {stars: abundances, stars: atmospheres, stars: Population II, globular clusters: general},
     year = 2010,
    month = jun,
   volume = 516,
      eid = {A55},
    pages = {A55},
      doi = {10.1051/0004-6361/200913451},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...516A..55C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Marina12,
   author = {{Rejkuba}, M.},
    title = "{Globular cluster luminosity function as distance indicator}",
  journal = {\apss},
archivePrefix = "arXiv",
   eprint = {1201.3936},
 primaryClass = "astro-ph.CO",
 keywords = {Globular clusters: general, Galaxies: distances and redshifts},
     year = 2012,
    month = sep,
   volume = 341,
    pages = {195-206},
      doi = {10.1007/s10509-012-0986-9},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012Ap%26SS.341..195R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Grebel16,
   author = {{Grebel}, E.~K.},
    title = "{Globular Clusters in the Local Group}",
 keywords = {Galaxy: globular clusters: general, Galaxy: halo, galaxies: star clusters, Local Group, galaxies: dwarfs, Magellanic Clouds, galaxies: abundances, galaxies: evolution, stellar content,},
booktitle = {Star Clusters and Black Holes in Galaxies across Cosmic Time},
     year = 2016,
   series = {IAU Symposium},
   volume = 312,
   editor = {{Meiron}, Y. and {Li}, S. and {Liu}, F.-K. and {Spurzem}, R.
	},
    month = feb,
    pages = {157-170},
      doi = {10.1017/S1743921315008078},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016IAUS..312..157G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McConnachie12,
   author = {{McConnachie}, A.~W.},
    title = "{The Observed Properties of Dwarf Galaxies in and around the Local Group}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1204.1562},
 keywords = {catalogs, galaxies: dwarf, galaxies: fundamental parameters, galaxies: general, galaxies: structure, Local Group},
     year = 2012,
    month = jul,
   volume = 144,
      eid = {4},
    pages = {4},
      doi = {10.1088/0004-6256/144/1/4},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012AJ....144....4M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Laporte17,
   author = {{Laporte}, C.~F.~P. and {Johnston}, K.~V. and {G{\'o}mez}, F.~A. and 
	{Garavito-Camargo}, N. and {Besla}, G.},
    title = "{The Influence of Sagittarius and the Large Magellanic Cloud on the Milky Way Galaxy}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1710.02538},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2017,
    month = oct,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017arXiv171002538L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Forbes18,
   author = {{Forbes}, D.~A. and {Bastian}, N. and {Gieles}, M. and {Crain}, R.~A. and 
	{Kruijssen}, J.~M.~D. and {Larsen}, S.~S. and {Ploeckinger}, S. and 
	{Agertz}, O. and {Trenti}, M. and {Ferguson}, A.~M.~N. and {Pfeffer}, J. and 
	{Gnedin}, O.~Y.},
    title = "{Globular cluster formation and evolution in the context of cosmological galaxy assembly: open questions}",
  journal = {Proceedings of the Royal Society of London Series A},
archivePrefix = "arXiv",
   eprint = {1801.05818},
     year = 2018,
    month = feb,
   volume = 474,
      eid = {20170616},
    pages = {20170616},
      doi = {10.1098/rspa.2017.0616},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2018RSPSA.47470616F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Forbes11,
   author = {{Forbes}, D.~A. and {Spitler}, L.~R. and {Strader}, J. and {Romanowsky}, A.~J. and 
	{Brodie}, J.~P. and {Foster}, C.},
    title = "{Evidence for two phases of galaxy formation from radial trends in the globular cluster system of NGC 1407}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1101.3575},
 keywords = {globular clusters: general, galaxies: formation, galaxies: individual: NGC 1407, galaxies: star clusters: general},
     year = 2011,
    month = jun,
   volume = 413,
    pages = {2943-2949},
      doi = {10.1111/j.1365-2966.2011.18373.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011MNRAS.413.2943F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HarrisGradients,
   author = {{Harris}, W.~E.},
    title = "{Globular Cluster Systems in Giant Ellipticals: The Mass/Metallicity Relation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0904.4208},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: elliptical and lenticular, cD, galaxies: star clusters, globular clusters: general},
     year = 2009,
    month = jul,
   volume = 699,
    pages = {254-280},
      doi = {10.1088/0004-637X/699/1/254},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009ApJ...699..254H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pota13,
   author = {{Pota}, V. and {Forbes}, D.~A. and {Romanowsky}, A.~J. and {Brodie}, J.~P. and 
	{Spitler}, L.~R. and {Strader}, J. and {Foster}, C. and {Arnold}, J.~A. and 
	{Benson}, A. and {Blom}, C. and {Hargis}, J.~R. and {Rhode}, K.~L. and 
	{Usher}, C.},
    title = "{The SLUGGS Survey: kinematics for over 2500 globular clusters in 12 early-type galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.4351},
 keywords = {globular clusters: general, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: star clusters: general},
     year = 2013,
    month = jan,
   volume = 428,
    pages = {389-420},
      doi = {10.1093/mnras/sts029},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.428..389P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LindegrenDR1,
   author = {{Lindegren}, L. and {Lammers}, U. and {Bastian}, U. and {Hern{\'a}ndez}, J. and 
	{Klioner}, S. and {Hobbs}, D. and {Bombrun}, A. and {Michalik}, D. and 
	{Ramos-Lerate}, M. and {Butkevich}, A. and {Comoretto}, G. and 
	{Joliet}, E. and {Holl}, B. and {Hutton}, A. and {Parsons}, P. and 
	{Steidelm{\"u}ller}, H. and {Abbas}, U. and {Altmann}, M. and 
	{Andrei}, A. and {Anton}, S. and {Bach}, N. and {Barache}, C. and 
	{Becciani}, U. and {Berthier}, J. and {Bianchi}, L. and {Biermann}, M. and 
	{Bouquillon}, S. and {Bourda}, G. and {Br{\"u}semeister}, T. and 
	{Bucciarelli}, B. and {Busonero}, D. and {Carlucci}, T. and 
	{Casta{\~n}eda}, J. and {Charlot}, P. and {Clotet}, M. and {Crosta}, M. and 
	{Davidson}, M. and {de Felice}, F. and {Drimmel}, R. and {Fabricius}, C. and 
	{Fienga}, A. and {Figueras}, F. and {Fraile}, E. and {Gai}, M. and 
	{Garralda}, N. and {Geyer}, R. and {Gonz{\'a}lez-Vidal}, J.~J. and 
	{Guerra}, R. and {Hambly}, N.~C. and {Hauser}, M. and {Jordan}, S. and 
	{Lattanzi}, M.~G. and {Lenhardt}, H. and {Liao}, S. and {L{\"o}ffler}, W. and 
	{McMillan}, P.~J. and {Mignard}, F. and {Mora}, A. and {Morbidelli}, R. and 
	{Portell}, J. and {Riva}, A. and {Sarasso}, M. and {Serraller}, I. and 
	{Siddiqui}, H. and {Smart}, R. and {Spagna}, A. and {Stampa}, U. and 
	{Steele}, I. and {Taris}, F. and {Torra}, J. and {van Reeven}, W. and 
	{Vecchiato}, A. and {Zschocke}, S. and {de Bruijne}, J. and 
	{Gracia}, G. and {Raison}, F. and {Lister}, T. and {Marchant}, J. and 
	{Messineo}, R. and {Soffel}, M. and {Osorio}, J. and {de Torres}, A. and 
	{O'Mullane}, W.},
    title = "{Gaia Data Release 1. Astrometry: one billion positions, two million proper motions and parallaxes}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1609.04303},
 keywords = {astrometry, parallaxes, proper motions, methods: data analysis, space vehicles: instruments, reference systems},
     year = 2016,
    month = nov,
   volume = 595,
      eid = {A4},
    pages = {A4},
      doi = {10.1051/0004-6361/201628714},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016A%26A...595A...4L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hayes18,
   author = {{Hayes}, C.~R. and {Majewski}, S.~R. and {Shetrone}, M. and 
	{Fern{\'a}ndez-Alvar}, E. and {Allende Prieto}, C. and {Schuster}, W.~J. and 
	{Carigi}, L. and {Cunha}, K. and {Smith}, V.~V. and {Sobeck}, J. and 
	{Almeida}, A. and {Beers}, T.~C. and {Carrera}, R. and {Fern{\'a}ndez-Trincado}, J.~G. and 
	{Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and {Geisler}, D. and {Lane}, R.~R. and 
	{Lucatello}, S. and {Matthews}, A.~M. and {Minniti}, D. and 
	{Nitschelm}, C. and {Tang}, B. and {Tissera}, P.~B. and {Zamora}, O.
	},
    title = "{Disentangling the Galactic Halo with APOGEE. I. Chemical and Kinematical Investigation of Distinct Metal-poor Populations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1711.05781},
 keywords = {Galaxy: disk, Galaxy: evolution, Galaxy: formation, Galaxy: halo, stars: abundances },
     year = 2018,
    month = jan,
   volume = 852,
      eid = {49},
    pages = {49},
      doi = {10.3847/1538-4357/aa9cec},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2018ApJ...852...49H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MichaelGES,
   author = {{Hayden}, M.~R. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Mikolaitis}, S. and {Guiglion}, G. and {Hill}, V. and {Gilmore}, G. and 
	{Randich}, S. and {Bayo}, A. and {Bensby}, T. and {Bergemann}, M. and 
	{Bragaglia}, A. and {Casey}, A. and {Costado}, M. and {Feltzing}, S. and 
	{Franciosini}, E. and {Hourihane}, A. and {Jofre}, P. and {Koposov}, S. and 
	{Kordopatis}, G. and {Lanzafame}, A. and {Lardo}, C. and {Lewis}, J. and 
	{Lind}, K. and {Magrini}, L. and {Monaco}, L. and {Morbidelli}, L. and 
	{Pancino}, E. and {Sacco}, G. and {Stonkute}, E. and {Worley}, C.~C. and 
	{Zwitter}, T.},
    title = "{The Gaia-ESO Survey: Churning through the Milky Way}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1711.05751},
 keywords = {Galaxy: kinematics and dynamics, Galaxy: disk, Galaxy: stellar content, Galaxy: structure},
     year = 2018,
    month = jan,
   volume = 609,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/201730412},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2018A%26A...609A..79H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Guillaume15,
   author = {{Guiglion}, G. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Kordopatis}, G. and {Hill}, V. and {Mikolaitis}, {\v S}. and 
	{Minchev}, I. and {Chiappini}, C. and {Wyse}, R.~F.~G. and {Gilmore}, G. and 
	{Randich}, S. and {Feltzing}, S. and {Bensby}, T. and {Flaccomio}, E. and 
	{Koposov}, S.~E. and {Pancino}, E. and {Bayo}, A. and {Costado}, M.~T. and 
	{Franciosini}, E. and {Hourihane}, A. and {Jofr{\'e}}, P. and 
	{Lardo}, C. and {Lewis}, J. and {Lind}, K. and {Magrini}, L. and 
	{Morbidelli}, L. and {Sacco}, G.~G. and {Ruchti}, G. and {Worley}, C.~C. and 
	{Zaggia}, S.},
    title = "{The Gaia-ESO Survey: New constraints on the Galactic disc velocity dispersion and its chemical dependencies}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1509.05271},
 keywords = {Galaxy: abundances, Galaxy: disk, Galaxy: kinematics and dynamics, Galaxy: stellar content, stars: abundances},
     year = 2015,
    month = nov,
   volume = 583,
      eid = {A91},
    pages = {A91},
      doi = {10.1051/0004-6361/201525883},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015A%26A...583A..91G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{IvanDispersion,
   author = {{Minchev}, I. and {Chiappini}, C. and {Martig}, M. and {Steinmetz}, M. and 
	{de Jong}, R.~S. and {Boeche}, C. and {Scannapieco}, C. and 
	{Zwitter}, T. and {Wyse}, R.~F.~G. and {Binney}, J.~J. and {Bland-Hawthorn}, J. and 
	{Bienaym{\'e}}, O. and {Famaey}, B. and {Freeman}, K.~C. and 
	{Gibson}, B.~K. and {Grebel}, E.~K. and {Gilmore}, G. and {Helmi}, A. and 
	{Kordopatis}, G. and {Lee}, Y.~S. and {Munari}, U. and {Navarro}, J.~F. and 
	{Parker}, Q.~A. and {Quillen}, A.~C. and {Reid}, W.~A. and {Siebert}, A. and 
	{Siviero}, A. and {Seabroke}, G. and {Watson}, F. and {Williams}, M.
	},
    title = "{A New Stellar Chemo-Kinematic Relation Reveals the Merger History of the Milky Way Disk}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1310.5145},
 keywords = {Galaxy: abundances, Galaxy: disk, Galaxy: evolution, Galaxy: formation, Galaxy: kinematics and dynamics, solar neighborhood},
     year = 2014,
    month = jan,
   volume = 781,
      eid = {L20},
    pages = {L20},
      doi = {10.1088/2041-8205/781/1/L20},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014ApJ...781L..20M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cristina2Infall,
   author = {{Chiappini}, C. and {Matteucci}, F. and {Gratton}, R.},
    title = "{The Chemical Evolution of the Galaxy: The Two-Infall Model}",
  journal = {\apj},
   eprint = {astro-ph/9609199},
 keywords = {ISM: individual (HH 1-2), ISM: Jets and Outflows, ISM: Molecules, ISM: Structure, Stars: Formation},
     year = 1997,
    month = mar,
   volume = 477,
    pages = {765-780},
      doi = {10.1086/303726},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1997ApJ...477..765C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tolstoy09,
   author = {{Tolstoy}, E. and {Hill}, V. and {Tosi}, M.},
    title = "{Star-Formation Histories, Abundances, and Kinematics of Dwarf Galaxies in the Local Group}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0904.4505},
 primaryClass = "astro-ph.CO",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {371-425},
      doi = {10.1146/annurev-astro-082708-101650},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009ARA%26A..47..371T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MatteucciGreggio,
   author = {{Matteucci}, F. and {Greggio}, L.},
    title = "{Relative roles of type I and II supernovae in the chemical enrichment of the interstellar gas}",
  journal = {\aap},
 keywords = {Chemical Evolution, Computational Astrophysics, Interstellar Gas, Nuclear Fusion, Supernovae, Galactic Evolution, Solar System, Stellar Evolution},
     year = 1986,
    month = jan,
   volume = 154,
    pages = {279-287},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1986A%26A...154..279M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Tinsley79,
   author = {{Tinsley}, B.~M.},
    title = "{Stellar lifetimes and abundance ratios in chemical evolution}",
  journal = {\apj},
 keywords = {Abundance, Chemical Evolution, Galactic Evolution, Life (Durability), Nuclear Fusion, Stellar Evolution, Carbon, Iron, Mass Ratios, Oxygen, Stellar Mass, Supernovae, Time Dependence, White Dwarf Stars},
     year = 1979,
    month = may,
   volume = 229,
    pages = {1046-1056},
      doi = {10.1086/157039},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1979ApJ...229.1046T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DeBoer15,
   author = {{de Boer}, T.~J.~L. and {Belokurov}, V. and {Koposov}, S.},
    title = "{The star formation history of the Sagittarius stream}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1505.00787},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: individual: Sagittarius, Local Group, galaxies: stellar content},
     year = 2015,
    month = aug,
   volume = 451,
    pages = {3489-3503},
      doi = {10.1093/mnras/stv946},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015MNRAS.451.3489D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{deBoer14,
   author = {{de Boer}, T.~J.~L. and {Belokurov}, V. and {Beers}, T.~C. and 
	{Lee}, Y.~S.},
    title = "{The {$\alpha$}-element knee of the Sagittarius stream}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1406.3352},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: individual: Sagittarius, Local Group, galaxies: stellar content},
     year = 2014,
    month = sep,
   volume = 443,
    pages = {658-663},
      doi = {10.1093/mnras/stu1176},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014MNRAS.443..658D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schuster12,
   author = {{Schuster}, W.~J. and {Moreno}, E. and {Nissen}, P.~E. and {Pichardo}, B.
	},
    title = "{Two distinct halo populations in the solar neighborhood. III. Evidence from stellar ages and orbital parameters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.4026},
 keywords = {stars: abundances, Galaxy: halo, stars: kinematics and dynamics, Galaxy: evolution},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A21},
    pages = {A21},
      doi = {10.1051/0004-6361/201118035},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...538A..21S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{MichaelAmbre,
   author = {{Hayden}, M.~R. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Mikolaitis}, S. and {Worley}, C.~C.},
    title = "{The AMBRE project: The thick thin disk and thin thick disk of the Milky Way}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1712.02358},
 keywords = {Galaxy: disk, Galaxy: structure, Galaxy: evolution, Galaxy: abundances, Galaxy: stellar content},
     year = 2017,
    month = nov,
   volume = 608,
      eid = {L1},
    pages = {L1},
      doi = {10.1051/0004-6361/201731494},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...608L...1H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kirby08,
   author = {{Kirby}, E.~N. and {Guhathakurta}, P. and {Sneden}, C.},
    title = "{Metallicity and Alpha-Element Abundance Measurement in Red Giant Stars from Medium-Resolution Spectra}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0804.3590},
 keywords = {globular clusters: individual: M13 M15 M71 M79 NGC 2419 NGC 7006 NGC 7492, stars: abundances},
     year = 2008,
    month = aug,
   volume = 682,
      eid = {1217-1233},
    pages = {1217-1233},
      doi = {10.1086/589627},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...682.1217K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mottini08,
   author = {{Mottini}, M. and {Wallerstein}, G. and {McWilliam}, A.},
    title = "{ARP 2 and Terzan 8: a Detailed Chemical Analysis}",
  journal = {\aj},
 keywords = {globular clusters: general, globular clusters: individual: Arp 2: Terzan 8},
     year = 2008,
    month = aug,
   volume = 136,
    pages = {614-620},
      doi = {10.1088/0004-6256/136/2/614},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008AJ....136..614M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kham14,
   author = {{Khamidullina}, D.~A. and {Sharina}, M.~E. and {Shimansky}, V.~V. and 
	{Davoust}, E.},
    title = "{Chemical abundances in the globular clusters NGC6229 and NGC6779}",
  journal = {Astrophysical Bulletin},
archivePrefix = "arXiv",
   eprint = {1502.02161},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy, abundances{\mdash}globular clusters, individual, NGC6229, NGC677},
     year = 2014,
    month = oct,
   volume = 69,
    pages = {409-426},
      doi = {10.1134/S199034131404004X},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014AstBu..69..409K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Linden17,
   author = {{Linden}, S.~T. and {Pryal}, M. and {Hayes}, C.~R. and {Troup}, N.~W. and 
	{Majewski}, S.~R. and {Andrews}, B.~H. and {Beers}, T.~C. and 
	{Carrera}, R. and {Cunha}, K. and {Fern{\'a}ndez-Trincado}, J.~G. and 
	{Frinchaboy}, P. and {Geisler}, D. and {Lane}, R.~R. and {Nitschelm}, C. and 
	{Pan}, K. and {Allende Prieto}, C. and {Roman-Lopes}, A. and 
	{Smith}, V.~V. and {Sobeck}, J. and {Tang}, B. and {Villanova}, S. and 
	{Zasowski}, G.},
    title = "{Timing the Evolution of the Galactic Disk with NGC 6791: An Open Cluster with Peculiar High-{$\alpha$} Chemistry as Seen by APOGEE}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1704.07305},
 keywords = {Galaxy: disk, Galaxy: evolution, Galaxy: stellar content, open clusters and associations: individual: NGC 6791, NGC 188, stars: abundances},
     year = 2017,
    month = jun,
   volume = 842,
      eid = {49},
    pages = {49},
      doi = {10.3847/1538-4357/aa6f17},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017ApJ...842...49L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{AlvaroGC,
   author = {{Rojas-Arriagada}, A. and {Zoccali}, M. and {V{\'a}squez}, S. and 
	{Ripepi}, V. and {Musella}, I. and {Marconi}, M. and {Grado}, A. and 
	{Limatola}, L.},
    title = "{High resolution spectroscopic analysis of seven giants in the bulge globular cluster NGC 6723}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1601.05736},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, Galaxy: bulge, globular clusters: general, globular clusters: individual: NGC 6723},
     year = 2016,
    month = mar,
   volume = 587,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201527351},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016A%26A...587A..95R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Omalley17,
   author = {{O'Malley}, E.~M. and {Knaizev}, A. and {McWilliam}, A. and 
	{Chaboyer}, B.},
    title = "{High-resolution Spectroscopic Abundances of Red Giant Branch Stars in NGC 6681}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1706.06962},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: individual: NGC 6681: M70, methods: observational, stars: abundances, stars: fundamental parameters},
     year = 2017,
    month = sep,
   volume = 846,
      eid = {23},
    pages = {23},
      doi = {10.3847/1538-4357/aa7b72},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017ApJ...846...23O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LeeCarney02,
   author = {{Lee}, J.-W. and {Carney}, B.~W.},
    title = "{Chemical Abundances of Three Metal-poor Globular Clusters (NGC 6287, NGC 6293, and NGC 6541) in the Inner Halo}",
  journal = {\aj},
   eprint = {astro-ph/0205393},
 keywords = {Galaxy: Halo, Galaxy: Globular Clusters: Individual: NGC Number: NGC 6287, globular clusters: individual (NGC 6293), globular clusters: individual (NGC 6541), Stars: Abundances},
     year = 2002,
    month = sep,
   volume = 124,
    pages = {1511-1527},
      doi = {10.1086/341948},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002AJ....124.1511L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Angie17,
   author = {{Bragaglia}, A. and {Carretta}, E. and {D'Orazi}, V. and {Sollima}, A. and 
	{Donati}, P. and {Gratton}, R.~G. and {Lucatello}, S.},
    title = "{NGC 6535: the lowest mass Milky Way globular cluster with a Na-O anti-correlation? Cluster mass and age in the multiple population context}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1708.07705},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: atmospheres, stars: Population II, open clusters and associations: individual: NGC 6535, globular clusters: general},
     year = 2017,
    month = nov,
   volume = 607,
      eid = {A44},
    pages = {A44},
      doi = {10.1051/0004-6361/201731526},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...607A..44B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hanke16,
   author = {{Hanke}, M. and {Koch}, A. and {Hansen}, C.~J. and {McWilliam}, A.
	},
    title = "{Insights into the chemical composition of the metal-poor Milky Way halo globular cluster <ASTROBJ>NGC 6426</ASTROBJ>}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1612.05989},
 keywords = {stars: abundances, Galaxy: abundances, Galaxy: evolution, Galaxy: halo, globular clusters: individual: NGC 6426},
     year = 2017,
    month = mar,
   volume = 599,
      eid = {A97},
    pages = {A97},
      doi = {10.1051/0004-6361/201629650},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...599A..97H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gratton87,
   author = {{Gratton}, R.~G.},
    title = "{The metal abundance of metal-rich globular clusters. III - NGC 288, NGC 362, NGC 5897, NGC 6352 and NGC 6362}",
  journal = {\aap},
 keywords = {Globular Clusters, Metallicity, Stellar Composition, Stellar Spectra, High Dispersion Spectrographs, Spectral Line Width, Spectrum Analysis, Stellar Atmospheres},
     year = 1987,
    month = jun,
   volume = 179,
    pages = {181-192},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1987A%26A...179..181G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Feltzing09,
   author = {{Feltzing}, S. and {Primas}, F. and {Johnson}, R.~A.},
    title = "{Stellar abundances and ages for metal-rich Milky Way globular clusters. Stellar parameters and elemental abundances for 9 HB stars in NGC 6352}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0810.4832},
 keywords = {galaxy: globular clusters: individual: NGC 6352, stars: horizontal-branch, stars: abundances},
     year = 2009,
    month = jan,
   volume = 493,
    pages = {913-930},
      doi = {10.1051/0004-6361:200810137},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...493..913F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Meszaros15,
   author = {{M{\'e}sz{\'a}ros}, S. and {Martell}, S.~L. and {Shetrone}, M. and 
	{Lucatello}, S. and {Troup}, N.~W. and {Bovy}, J. and {Cunha}, K. and 
	{Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and {Overbeek}, J.~C. and 
	{Allende Prieto}, C. and {Beers}, T.~C. and {Frinchaboy}, P.~M. and 
	{Garc{\'{\i}}a P{\'e}rez}, A.~E. and {Hearty}, F.~R. and {Holtzman}, J. and 
	{Majewski}, S.~R. and {Nidever}, D.~L. and {Schiavon}, R.~P. and 
	{Schneider}, D.~P. and {Sobeck}, J.~S. and {Smith}, V.~V. and 
	{Zamora}, O. and {Zasowski}, G.},
    title = "{Exploring Anticorrelations and Light Element Variations in Northern Globular Clusters Observed by the APOGEE Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1501.05127},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: AGB and post-AGB, stars: chemically peculiar, stars: evolution},
     year = 2015,
    month = may,
   volume = 149,
      eid = {153},
    pages = {153},
      doi = {10.1088/0004-6256/149/5/153},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015AJ....149..153M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Johnson16,
   author = {{Johnson}, C.~I. and {Caldwell}, N. and {Rich}, R.~M. and {Pilachowski}, C.~A. and 
	{Hsyu}, T.},
    title = "{The Chemical Composition of Red Giant Branch Stars in the Galactic Globular Clusters NGC 6342 and NGC 6366}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1606.08491},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: general, globular clusters: individual: NGC 6342, NGC 6366, stars: abundances},
     year = 2016,
    month = jul,
   volume = 152,
      eid = {21},
    pages = {21},
      doi = {10.3847/0004-6256/152/1/21},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016AJ....152...21J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Johnson17,
   author = {{Johnson}, C.~I. and {Caldwell}, N. and {Rich}, R.~M. and {Mateo}, M. and 
	{Bailey}, III, J.~I. and {Olszewski}, E.~W. and {Walker}, M.~G.
	},
    title = "{Chemical Complexity in the Eu-enhanced Monometallic Globular NGC 5986}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1705.10840},
 primaryClass = "astro-ph.SR",
 keywords = {globular clusters: general, globular clusters: individual: NGC 5986, stars: abundances},
     year = 2017,
    month = jun,
   volume = 842,
      eid = {24},
    pages = {24},
      doi = {10.3847/1538-4357/aa7414},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017ApJ...842...24J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bulbo17,
   author = {{Recio-Blanco}, A. and {Rojas-Arriagada}, A. and {de Laverny}, P. and 
	{Mikolaitis}, S. and {Hill}, V. and {Zoccali}, M. and {Fern{\'a}ndez-Trincado}, J.~G. and 
	{Robin}, A.~C. and {Babusiaux}, C. and {Gilmore}, G. and {Randich}, S. and 
	{Alfaro}, E. and {Allende Prieto}, C. and {Bragaglia}, A. and 
	{Carraro}, G. and {Jofr{\'e}}, P. and {Lardo}, C. and {Monaco}, L. and 
	{Morbidelli}, L. and {Zaggia}, S.},
    title = "{The Gaia-ESO Survey: Low-{$\alpha$} element stars in the Galactic bulge}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1702.04500},
 keywords = {Galaxy: bulge, Galaxy: abundances, Galaxy: stellar content},
     year = 2017,
    month = jun,
   volume = 602,
      eid = {L14},
    pages = {L14},
      doi = {10.1051/0004-6361/201630220},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...602L..14R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lamb15,
   author = {{Lamb}, M.~P. and {Venn}, K.~A. and {Shetrone}, M.~D. and {Sakari}, C.~M. and 
	{Pritzl}, B.~J.},
    title = "{Chemical abundances in the globular clusters NGC 5024 and NGC 5466 from optical and infrared spectroscopy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1412.5210},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: spectroscopic, stars: abundances, globular clusters: individual: (NGC 5024), globular clusters: individual: (NGC 5466)},
     year = 2015,
    month = mar,
   volume = 448,
    pages = {42-58},
      doi = {10.1093/mnras/stu2674},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015MNRAS.448...42L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Marino15,
   author = {{Marino}, A.~F. and {Milone}, A.~P. and {Karakas}, A.~I. and 
	{Casagrande}, L. and {Yong}, D. and {Shingles}, L. and {Da Costa}, G. and 
	{Norris}, J.~E. and {Stetson}, P.~B. and {Lind}, K. and {Asplund}, M. and 
	{Collet}, R. and {Jerjen}, H. and {Sbordone}, L. and {Aparicio}, A. and 
	{Cassisi}, S.},
    title = "{Iron and s-elements abundance variations in NGC 5286: comparison with `anomalous' globular clusters and Milky Way satellites}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1502.07438},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, globular clusters: general, globular clusters: individual: NGC 5286},
     year = 2015,
    month = jun,
   volume = 450,
    pages = {815-845},
      doi = {10.1093/mnras/stv420},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015MNRAS.450..815M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Marino11,
   author = {{Marino}, A.~F. and {Sneden}, C. and {Kraft}, R.~P. and {Wallerstein}, G. and 
	{Norris}, J.~E. and {da Costa}, G. and {Milone}, A.~P. and {Ivans}, I.~I. and 
	{Gonzalez}, G. and {Fulbright}, J.~P. and {Hilker}, M. and {Piotto}, G. and 
	{Zoccali}, M. and {Stetson}, P.~B.},
    title = "{The two metallicity groups of the globular cluster M 22: a chemical perspective}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1105.1523},
 primaryClass = "astro-ph.SR",
 keywords = {techniques: spectroscopic, stars: abundances, stars: Population II, globular clusters: individual: M 22 (NGC 6656)},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A8},
    pages = {A8},
      doi = {10.1051/0004-6361/201116546},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...532A...8M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Filler12,
   author = {{Filler}, D. and {Ivans}, I.~I. and {Simmerer}, J.},
    title = "{Galactic Globular Cluster NGC1261: ``Young'', Low-alpha and Star-to-Star Abundance Variations In Na-O?}",
booktitle = {American Astronomical Society Meeting Abstracts \#219},
     year = 2012,
   series = {American Astronomical Society Meeting Abstracts},
   volume = 219,
    month = jan,
      eid = {152.05},
    pages = {152.05},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012AAS...21915205F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Luca15,
   author = {{Sbordone}, L. and {Monaco}, L. and {Moni Bidin}, C. and {Bonifacio}, P. and 
	{Villanova}, S. and {Bellazzini}, M. and {Ibata}, R. and {Chiba}, M. and 
	{Geisler}, D. and {Caffau}, E. and {Duffau}, S.},
    title = "{Chemical abundances of giant stars in <ASTROBJ>NGC 5053</ASTROBJ> and <ASTROBJ>NGC 5634</ASTROBJ>, two globular clusters associated with the Sagittarius dwarf spheroidal galaxy?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1505.01487},
 keywords = {Galaxy: abundances, globular clusters: individual: NGC 5053, globular clusters: individual: NGC 5634, galaxies: active, stars: abundances, galaxies: individual: Sgr dSph},
     year = 2015,
    month = jul,
   volume = 579,
      eid = {A104},
    pages = {A104},
      doi = {10.1051/0004-6361/201425509},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015A%26A...579A.104S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Luca05,
   author = {{Sbordone}, L. and {Bonifacio}, P. and {Marconi}, G. and {Buonanno}, R. and 
	{Zaggia}, S.},
    title = "{Family ties: Abundances in Terzan 7, a Sgr dSph globular cluster}",
  journal = {\aap},
   eprint = {astro-ph/0505307},
 keywords = {stars: abundances, stars: atmospheres, Galaxy: globular clusters: individual: Terzan 7, galaxies: abundances, galaxies: individual: Terzan 7, galaxies: evolution},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {905-910},
      doi = {10.1051/0004-6361:20042315},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005A%26A...437..905S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sandro16,
   author = {{Villanova}, S. and {Monaco}, L. and {Moni Bidin}, C. and {Assmann}, P.
	},
    title = "{A spectroscopic study of the globular Cluster NGC 4147}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1605.03408},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, globular clusters: individual: NGC4147},
     year = 2016,
    month = aug,
   volume = 460,
    pages = {2351-2359},
      doi = {10.1093/mnras/stw1146},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016MNRAS.460.2351V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sandro13,
   author = {{Villanova}, S. and {Geisler}, D. and {Carraro}, G. and {Moni Bidin}, C. and 
	{Mu{\~n}oz}, C.},
    title = "{Ruprecht 106: The First Single Population Globular Cluster?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1310.5900},
 keywords = {globular clusters: general, globular clusters: individual: Ruprecht 106},
     year = 2013,
    month = dec,
   volume = 778,
      eid = {186},
    pages = {186},
      doi = {10.1088/0004-637X/778/2/186},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...778..186V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eu10,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R.~G. and 
	{Lucatello}, S. and {Bellazzini}, M. and {Catanzaro}, G. and 
	{Leone}, F. and {Momany}, Y. and {Piotto}, G. and {D'Orazi}, V.
	},
    title = "{Detailed abundances of a large sample of giant stars in M 54 and in the Sagittarius nucleus}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1006.5866},
 keywords = {stars: abundances, stars: atmospheres, stars: Population II, globular clusters: individual: NGC 6715 (M 54), globular clusters: individual: NGC 5139 ({$\omega$} Cen), globular clusters: general},
     year = 2010,
    month = sep,
   volume = 520,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201014924},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...520A..95C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Eu14b,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R.~G. and 
	{D'Orazi}, V. and {Lucatello}, S. and {Momany}, Y. and {Sollima}, A. and 
	{Bellazzini}, M. and {Catanzaro}, G. and {Leone}, F.},
    title = "{The extreme chemistry of multiple stellar populations in the metal-poor globular cluster NGC 4833}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1401.7325},
 keywords = {stars: abundances, stars: atmospheres, stars: Population II, globular clusters: general, globular clusters: individual: NGC 4833},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A60},
    pages = {A60},
      doi = {10.1051/0004-6361/201323321},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...564A..60C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eu14a,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R.~G. and 
	{D'Orazi}, V. and {Lucatello}, S. and {Sollima}, A.},
    title = "{Terzan 8: a Sagittarius-flavoured globular cluster}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1311.2589},
 keywords = {stars: abundances, stars: Population II, globular clusters: general, globular clusters: individual: Terzan 8, stars: atmospheres},
     year = 2014,
    month = jan,
   volume = 561,
      eid = {A87},
    pages = {A87},
      doi = {10.1051/0004-6361/201322676},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...561A..87C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eu13,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R.~G. and 
	{Lucatello}, S. and {D'Orazi}, V. and {Bellazzini}, M. and {Catanzaro}, G. and 
	{Leone}, F. and {Momany}, Y. and {Sollima}, A.},
    title = "{NGC 362: another globular cluster with a split red giant branch}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.4085},
 keywords = {stars: Population II, globular clusters: general, stars: abundances, stars: atmospheres, globular clusters: individual: NGC 362},
     year = 2013,
    month = sep,
   volume = 557,
      eid = {A138},
    pages = {A138},
      doi = {10.1051/0004-6361/201321905},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26A...557A.138C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eu11,
   author = {{Carretta}, E. and {Lucatello}, S. and {Gratton}, R.~G. and 
	{Bragaglia}, A. and {D'Orazi}, V.},
    title = "{Multiple stellar populations in the globular cluster NGC 1851}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1106.3174},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: atmospheres, globular clusters: general, globular clusters: individual: NGC 1851, stars: Population II},
     year = 2011,
    month = sep,
   volume = 533,
      eid = {A69},
    pages = {A69},
      doi = {10.1051/0004-6361/201117269},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...533A..69C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cohen04,
   author = {{Cohen}, J.~G.},
    title = "{Palomar 12 as a Part of the Sagittarius Stream: The Evidence from Abundance Ratios}",
  journal = {\aj},
   eprint = {astro-ph/0311187},
 keywords = {Galaxy: Globular Clusters: General, Galaxy: Globular Clusters: Individual: Name: Palomar 12, Galaxies: Individual: Name: Sagittarius Dwarf Spheroidal, Stars: Abundances},
     year = 2004,
    month = mar,
   volume = 127,
    pages = {1545-1554},
      doi = {10.1086/382104},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004AJ....127.1545C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EugenioUVES,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R. and {Lucatello}, S.
	},
    title = "{Na-O anticorrelation and HB. VIII. Proton-capture elements and metallicities in 17 globular clusters from UVES spectra}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0909.2941},
 keywords = {stars: abundances, stars: atmospheres, stars: population II, Galaxy: globular clusters: general},
     year = 2009,
    month = oct,
   volume = 505,
    pages = {139-155},
      doi = {10.1051/0004-6361/200912097},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...505..139C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dinescu07,
   author = {{Casetti-Dinescu}, D.~I. and {Girard}, T.~M. and {Herrera}, D. and 
	{van Altena}, W.~F. and {L{\'o}pez}, C.~E. and {Castillo}, D.~J.
	},
    title = "{Space Velocities of Southern Globular Clusters. V. A Low Galactic Latitude Sample}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0705.3438},
 keywords = {astrometry, globular clusters: individual: NGC 2808: NGC 3201: NGC 4372: NGC 4833: NGC 5927: NGC 5986, surveys},
     year = 2007,
    month = jul,
   volume = 134,
    pages = {195-204},
      doi = {10.1086/518507},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007AJ....134..195C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harris,
   author = {{Harris}, W.~E.},
    title = "{A Catalog of Parameters for Globular Clusters in the Milky Way}",
  journal = {\aj},
 keywords = {GLOBULAR CLUSTERS: GENERAL, CATALOGS},
     year = 1996,
    month = oct,
   volume = 112,
    pages = {1487},
      doi = {10.1086/118116},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1996AJ....112.1487H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VdbMakey04,
   author = {{van den Bergh}, S. and {Mackey}, A.~D.},
    title = "{Globular clusters and the formation of the outer Galactic halo}",
  journal = {\mnras},
   eprint = {astro-ph/0407346},
 keywords = {Galaxy: formation, globular clusters: general, Galaxy: halo, Magellanic Clouds},
     year = 2004,
    month = nov,
   volume = 354,
    pages = {713-719},
      doi = {10.1111/j.1365-2966.2004.08228.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.354..713V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Sharina05,
   author = {{Sharina}, M.~E. and {Puzia}, T.~H. and {Makarov}, D.~I.},
    title = "{Hubble Space Telescope imaging of globular cluster candidates in low surface brightness dwarf galaxies}",
  journal = {\aap},
   eprint = {astro-ph/0505624},
 keywords = {galaxies: dwarf, galaxies: star clusters},
     year = 2005,
    month = oct,
   volume = 442,
    pages = {85-95},
      doi = {10.1051/0004-6361:20052921},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...442...85S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VdB06,
      author = {{van den Bergh}, S.},
    title = "{Globular Clusters in Dwarf Galaxies}",
  journal = {\aj},
   eprint = {astro-ph/0509811},
 keywords = {Galaxies: Dwarf, Galaxies: Star Clusters, Galaxy: Globular Clusters: General},
     year = 2006,
    month = jan,
   volume = 131,
    pages = {304-311},
      doi = {10.1086/498688},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006AJ....131..304V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dinescu99b,
   author = {{Dinescu}, D.~I. and {van Altena}, W.~F. and {Girard}, T.~M. and 
	{L{\'o}pez}, C.~E.},
    title = "{Space Velocities of Southern Globular Clusters. II. New Results for 10 Clusters}",
  journal = {\aj},
 keywords = {ASTROMETRY, GALAXY: GLOBULAR CLUSTERS: GENERAL, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 1904, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 2298, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 4590, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 5139, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 5897, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 6093, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 6121, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 6144, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 6809, GALAXY: GLOBULAR CLUSTERS: INDIVIDUAL: NGC NUMBER: NGC 7099},
     year = 1999,
    month = jan,
   volume = 117,
    pages = {277-285},
      doi = {10.1086/300699},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999AJ....117..277D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dinescu99a,
   author = {{Dinescu}, D.~I. and {Girard}, T.~M. and {van Altena}, W.~F.
	},
    title = "{Space Velocities of Globular Clusters. III. Cluster Orbits and Halo Substructure}",
  journal = {\aj},
 keywords = {GALAXY: HALO, GALAXY: STRUCTURE, GALAXY: GLOBULAR CLUSTERS: GENERAL},
     year = 1999,
    month = apr,
   volume = 117,
    pages = {1792-1815},
      doi = {10.1086/300807},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999AJ....117.1792D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SarunasAmbre,
   author = {{Mikolaitis}, {\v S}. and {de Laverny}, P. and {Recio-Blanco}, A. and 
	{Hill}, V. and {Worley}, C.~C. and {de Pascale}, M.},
    title = "{The AMBRE project: Iron-peak elements in the solar neighbourhood}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1612.07622},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy, stars: abundances, Galaxy: stellar content, star: abundances},
     year = 2017,
    month = apr,
   volume = 600,
      eid = {A22},
    pages = {A22},
      doi = {10.1051/0004-6361/201629629},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...600A..22M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Harps,
   author = {{De Pascale}, M. and {Worley}, C.~C. and {de Laverny}, P. and 
	{Recio-Blanco}, A. and {Hill}, V. and {Bijaoui}, A.},
    title = "{The AMBRE project: Parameterisation of FGK-type stars from the ESO:HARPS archived spectra}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1409.2258},
 primaryClass = "astro-ph.IM",
 keywords = {astronomical databases: miscellaneous, stars: fundamental parameters, stars: abundances, techniques: spectroscopic, methods: data analysis},
     year = 2014,
    month = oct,
   volume = 570,
      eid = {A68},
    pages = {A68},
      doi = {10.1051/0004-6361/201423767},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...570A..68D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{EugenioScale,
   author = {{Carretta}, E. and {Bragaglia}, A. and {Gratton}, R. and {D'Orazi}, V. and 
	{Lucatello}, S.},
    title = "{Intrinsic iron spread and a new metallicity scale for globular clusters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0910.0675},
 keywords = {stars: abundances, stars: atmospheres, stars: population II, globular clusters: general},
     year = 2009,
    month = dec,
   volume = 508,
    pages = {695-706},
      doi = {10.1051/0004-6361/200913003},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...508..695C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ambre,
   author = {{de Laverny}, P. and {Recio-Blanco}, A. and {Worley}, C.~C. and 
	{Plez}, B.},
    title = "{The AMBRE project: A new synthetic grid of high-resolution FGKM stellar spectra}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1205.2270},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, stars: fundamental parameters, stars: abundances, astronomical databases: miscellaneous, surveys},
     year = 2012,
    month = aug,
   volume = 544,
      eid = {A126},
    pages = {A126},
      doi = {10.1051/0004-6361/201219330},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...544A.126D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{V13,
   author = {{VandenBerg}, D.~A. and {Brogaard}, K. and {Leaman}, R. and 
	{Casagrande}, L.},
    title = "{The Ages of 55 Globular Clusters as Determined Using an Improved $\backslash$Delta V\^{}HB\_TO Method along with Color-Magnitude Diagram Constraints, and Their Implications for Broader Issues}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1308.2257},
 primaryClass = "astro-ph.GA",
 keywords = {globular clusters: general, stars: abundances, stars: evolution, stars: interiors, stars: Population II},
     year = 2013,
    month = oct,
   volume = 775,
      eid = {134},
    pages = {134},
      doi = {10.1088/0004-637X/775/2/134},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...775..134V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Leaman13,
   author = {{Leaman}, R. and {VandenBerg}, D.~A. and {Mendel}, J.~T.},
    title = "{The bifurcated age-metallicity relation of Milky Way globular clusters and its implications for the accretion history of the galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1309.0822},
 keywords = {Galaxy: formation, globular clusters: general, galaxies: dwarf},
     year = 2013,
    month = nov,
   volume = 436,
    pages = {122-135},
      doi = {10.1093/mnras/stt1540},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.436..122L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Forbes10,
   author = {{Forbes}, D.~A. and {Bridges}, T.},
    title = "{Accreted versus in situ Milky Way globular clusters}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1001.4289},
 keywords = {Galaxy: evolution, Galaxy: formation, globular clusters: general, Galaxy: halo},
     year = 2010,
    month = may,
   volume = 404,
    pages = {1203-1214},
      doi = {10.1111/j.1365-2966.2010.16373.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010MNRAS.404.1203F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dotter11,
   author = {{Dotter}, A. and {Sarajedini}, A. and {Anderson}, J.},
    title = "{Globular Clusters in the Outer Galactic Halo: New Hubble Space Telescope/Advanced Camera for Surveys Imaging of Six Globular Clusters and the Galactic Globular Cluster Age-metallicity Relation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.4307},
 keywords = {Galaxy: formation, globular clusters: general},
     year = 2011,
    month = sep,
   volume = 738,
      eid = {74},
    pages = {74},
      doi = {10.1088/0004-637X/738/1/74},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011ApJ...738...74D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}

@ARTICLE{Antonio09,
   author = {{Mar{\'{\i}}n-Franch}, A. and {Aparicio}, A. and {Piotto}, G. and 
	{Rosenberg}, A. and {Chaboyer}, B. and {Sarajedini}, A. and 
	{Siegel}, M. and {Anderson}, J. and {Bedin}, L.~R. and {Dotter}, A. and 
	{Hempel}, M. and {King}, I. and {Majewski}, S. and {Milone}, A.~P. and 
	{Paust}, N. and {Reid}, I.~N.},
    title = "{The ACS Survey of Galactic Globular Clusters. VII. Relative Ages}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0812.4541},
 keywords = {Galaxy: evolution, Galaxy: formation, globular clusters: general},
     year = 2009,
    month = apr,
   volume = 694,
    pages = {1498-1516},
      doi = {10.1088/0004-637X/694/2/1498},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009ApJ...694.1498M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VandenBerg00,
   author = {{VandenBerg}, D.~A.},
    title = "{Models for Old, Metal-Poor Stars with Enhanced {$\alpha$}-Element Abundances. II. Their Implications for the Ages of the Galaxy's Globular Clusters and Field Halo Stars}",
  journal = {\apjs},
 keywords = {Galaxy: Globular Clusters: General, Stars: Evolution, Stars: Interiors, Stars: Population II},
     year = 2000,
    month = jul,
   volume = 129,
    pages = {315-352},
      doi = {10.1086/313404},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2000ApJS..129..315V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Alfred99,
   author = {{Rosenberg}, A. and {Saviane}, I. and {Piotto}, G. and {Aparicio}, A.
	},
    title = "{Galactic Globular Cluster Relative Ages}",
  journal = {\aj},
   eprint = {astro-ph/9907394},
 keywords = {STARS: COLOR-MAGNITUDE DIAGRAMS, GALAXY: EVOLUTION, GALAXY: FORMATION, GALAXY: GLOBULAR CLUSTERS: GENERAL, STARS: POPULATION II},
     year = 1999,
    month = nov,
   volume = 118,
    pages = {2306-2320},
      doi = {10.1086/301089},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999AJ....118.2306R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SalarisWeiss02,
   author = {{Salaris}, M. and {Weiss}, A.},
    title = "{Homogeneous age dating of 55 Galactic globular clusters. Clues to the Galaxy formation mechanisms}",
  journal = {\aap},
   eprint = {astro-ph/0204410},
 keywords = {Galaxy: formation, Galaxy: halo, globular clusters: general, stars: Hertzsprung-Russell diagram, stars: Population II},
     year = 2002,
    month = jun,
   volume = 388,
    pages = {492-503},
      doi = {10.1051/0004-6361:20020554},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002A%26A...388..492S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Buonanno98,
   author = {{Buonanno}, R. and {Corsi}, C.~E. and {Pulone}, L. and {Fusi Pecci}, F. and 
	{Bellazzini}, M.},
    title = "{On the relative ages of galactic globular clusters. A new observable, a semi-empirical calibration and problems with the theoretical isochrones}",
  journal = {\aap},
 keywords = {STARS: EVOLUTION, STARS: HORIZONTAL-BRANCH, STARS: POPULATION II, GLOBULAR CLUSTERS: GENERAL},
     year = 1998,
    month = may,
   volume = 333,
    pages = {505-523},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1998A%26A...333..505B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Francesca,
   author = {{De Angeli}, F. and {Piotto}, G. and {Cassisi}, S. and {Busso}, G. and 
	{Recio-Blanco}, A. and {Salaris}, M. and {Aparicio}, A. and 
	{Rosenberg}, A.},
    title = "{Galactic Globular Cluster Relative Ages}",
  journal = {\aj},
   eprint = {astro-ph/0503594},
 keywords = {Galaxy: Evolution, Galaxy: Formation, Galaxy: Globular Clusters: General},
     year = 2005,
    month = jul,
   volume = 130,
    pages = {116-125},
      doi = {10.1086/430723},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005AJ....130..116D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barbuy2009,
   author = {{Barbuy}, B. and {Zoccali}, M. and {Ortolani}, S. and {Hill}, V. and 
	{Minniti}, D. and {Bica}, E. and {Renzini}, A. and {G{\'o}mez}, A.
	},
    title = "{VLT-FLAMES analysis of 8 giants in the bulge metal-poor globular cluster NGC 6522: oldest cluster in the Galaxy?. Analysis of 8 giants in NGC 6522}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0908.3603},
 keywords = {stars: abundances, galaxy: bulge, galaxy: globular clusters: individual: NGC 6522},
     year = 2009,
    month = nov,
   volume = 507,
    pages = {405-415},
      doi = {10.1051/0004-6361/200912748},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...507..405B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{AnaElia13,
   author = {{Garc{\'{\i}}a P{\'e}rez}, A.~E. and {Cunha}, K. and {Shetrone}, M. and 
	{Majewski}, S.~R. and {Johnson}, J.~A. and {Smith}, V.~V. and 
	{Schiavon}, R.~P. and {Holtzman}, J. and {Nidever}, D. and {Zasowski}, G. and 
	{Allende Prieto}, C. and {Beers}, T.~C. and {Bizyaev}, D. and 
	{Ebelke}, G. and {Eisenstein}, D.~J. and {Frinchaboy}, P.~M. and 
	{Girardi}, L. and {Hearty}, F.~R. and {Malanushenko}, E. and 
	{Malanushenko}, V. and {Meszaros}, S. and {O'Connell}, R.~W. and 
	{Oravetz}, D. and {Pan}, K. and {Robin}, A.~C. and {Schneider}, D.~P. and 
	{Schultheis}, M. and {Skrutskie}, M.~F. and {Simmonsand}, A. and 
	{Wilson}, J.~C.},
    title = "{Very Metal-poor Stars in the Outer Galactic Bulge Found by the APOGEE Survey}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1301.1367},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: atmospheres, Galaxy: center, Galaxy: structure},
     year = 2013,
    month = apr,
   volume = 767,
      eid = {L9},
    pages = {L9},
      doi = {10.1088/2041-8205/767/1/L9},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...767L...9G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ness14,
   author = {{Ness}, M. and {Asplund}, M. and {Casey}, A.~R.},
    title = "{NGC 6522: a typical globular cluster in the Galactic bulge without signatures of rapidly rotating Population III stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1408.0290},
 keywords = {stars: abundances, stars: Population III, Galaxy: abundances, Galaxy: bulge, globular clusters: general},
     year = 2014,
    month = dec,
   volume = 445,
    pages = {2994-2998},
      doi = {10.1093/mnras/stu2144},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014MNRAS.445.2994N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McWilliamRich,
   author = {{McWilliam}, A. and {Rich}, R.~M.},
    title = "{The first detailed abundance analysis of Galactic bulge K giants in Baade's window}",
  journal = {\apjs},
 keywords = {Abundance, G Stars, Galactic Bulge, Giant Stars, Globular Clusters, Infrared Spectra, K Stars, Metallic Stars, Metallicity, Echelle Gratings, Infrared Astronomy, Stellar Mass, Stellar Temperature, Temperature Scales},
     year = 1994,
    month = apr,
   volume = 91,
    pages = {749-791},
      doi = {10.1086/191954},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1994ApJS...91..749M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Manu17,
   author = {{Zoccali}, M. and {Vasquez}, S. and {Gonzalez}, O.~A. and {Valenti}, E. and 
	{Rojas-Arriagada}, A. and {Minniti}, J. and {Rejkuba}, M. and 
	{Minniti}, D. and {McWilliam}, A. and {Babusiaux}, C. and {Hill}, V. and 
	{Renzini}, A.},
    title = "{The GIRAFFE Inner Bulge Survey (GIBS) III. Metallicity distributions and kinematics of 26 Galactic bulge fields}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.09174},
 keywords = {Astrophysics - Astrophysics of Galaxies},
     year = 2016,
    month = oct,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016arXiv161009174Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GESRandich,
   author = {{Randich}, S. and {Gilmore}, G. and {Gaia-ESO Consortium}},
    title = "{The Gaia-ESO Large Public Spectroscopic Survey}",
  journal = {The Messenger},
     year = 2013,
    month = dec,
   volume = 154,
    pages = {47-49},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013Msngr.154...47R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{JoseModel,
author = {{Fern{\'a}ndez-Trincado}, J.~G. and {Robin}, A.~C. and {Moreno}, E. and 
	{Schiavon}, R.~P. and {Garc{\'{\i}}a P{\'e}rez}, A.~E. and {Vieira}, K. and 
	{Cunha}, K. and {Zamora}, O. and {Sneden}, C. and {Souto}, D. and 
	{Carrera}, R. and {Johnson}, J.~A. and {Shetrone}, M. and {Zasowski}, G. and 
	{Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and {Majewski}, S.~R. and 
	{Reyl{\'e}}, C. and {Blanco-Cuaresma}, S. and {Martinez-Medina}, L.~A. and 
	{P{\'e}rez-Villegas}, A. and {Valenzuela}, O. and {Pichardo}, B. and 
	{Meza}, A. and {M{\'e}sz{\'a}ros}, S. and {Sobeck}, J. and {Geisler}, D. and 
	{Anders}, F. and {Schultheis}, M. and {Tang}, B. and {Roman-Lopes}, A. and 
	{Mennickent}, R.~E. and {Pan}, K. and {Nitschelm}, C. and {Allard}, F.
	},
    title = "{Discovery of a Metal-poor Field Giant with a Globular Cluster Second-generation Abundance Pattern}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1604.01279},
 keywords = {globular clusters: general, stars: abundances, stars: Population II},
     year = 2016,
    month = dec,
   volume = 833,
      eid = {132},
    pages = {132},
      doi = {10.3847/1538-4357/833/2/132},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016ApJ...833..132F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mathias16,
   author = {{Schultheis}, M. and {Rojas-Arriagada}, A. and {Garc\'ia P\'erez}, A. E. and {Jonsson}, H. and {Hayden}, M. and
            {Nandakumar}, G. and {Cunha}, K. and {APOGEE}},
    title = "{APOGEE et BW}",
  journal = {\aap},
     year = 2016,
     pages = {submitted}
}


@ARTICLE{AlvaroDisc,
   author = {{Rojas-Arriagada}, A. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Schultheis}, M. d {Guiglion}, G. and {Mikolaitis}, {\v S}. and 
	{Kordopatis}, G. and {Hill}, V. and {Gilmore}, G. and {Randich}, S. and 
	{Alfaro}, E.~J. and {Bensby}, T. and {Koposov}, S.~E. and {Costado}, M.~T. and 
	{Franciosini}, E. and {Hourihane}, A. and {Jofr{\'e}}, P. and 
	{Lardo}, C. and {Lewis}, J. and {Lind}, K. and {Magrini}, L. and 
	{Monaco}, L. and {Morbidelli}, L. and {Sacco}, G.~G. and {Worley}, C.~C. and 
	{Zaggia}, S. and {Chiappini}, C.},
    title = "{The Gaia-ESO Survey: Separating disk chemical substructures with cluster models. Evidence of a separate evolution in the metal-poor thin disk}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1512.03835},
 keywords = {Galaxy: formation, Galaxy: abundances, Galaxy: stellar content, stars: abundances},
     year = 2016,
    month = feb,
   volume = 586,
      eid = {A39},
    pages = {A39},
      doi = {10.1051/0004-6361/201526969},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016A%26A...586A..39R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sbordone07,
   author = {{Sbordone}, L. and {Bonifacio}, P. and {Buonanno}, R. and {Marconi}, G. and 
	{Monaco}, L. and {Zaggia}, S.},
    title = "{The exotic chemical composition of the Sagittarius dwarf spheroidal galaxy}",
  journal = {\aap},
   eprint = {astro-ph/0612125},
 keywords = {stars: abundances, stars: atmospheres, Galaxy: abundances, galaxies: dwarf, galaxies: individual: Sgr dSph, Galaxy: globular clusters: individual: Terzan 7},
     year = 2007,
    month = apr,
   volume = 465,
    pages = {815-824},
      doi = {10.1051/0004-6361:20066385},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...465..815S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McWilliam13,
   author = {{McWilliam}, A. and {Wallerstein}, G. and {Mottini}, M.},
    title = "{Chemistry of the Sagittarius Dwarf Galaxy: A Top-light Initial Mass Function, Outflows, and the R-process}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1309.2974},
 keywords = {galaxies: abundances, galaxies: dwarf, stars: abundances, stars: late-type},
     year = 2013,
    month = dec,
   volume = 778,
      eid = {149},
    pages = {149},
      doi = {10.1088/0004-637X/778/2/149},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...778..149M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sumi,
   author = {{Sumi}, T. and {Wu}, X. and {Udalski}, A. and {Szyma{\'n}ski}, M. and 
	{Kubiak}, M. and {Pietrzy{\'n}ski}, G. and {Soszy{\'n}ski}, I. and 
	{Wo{\'z}niak}, P. and {{\.Z}ebru{\'n}}, K. and {Szewczyk}, O. and 
	{Wyrzykowski}, {\L}.},
    title = "{The Optical Gravitational Lensing Experiment: catalogue of stellar proper motions in the OGLE-II Galactic bulge fields}",
  journal = {\mnras},
   eprint = {astro-ph/0305315},
 keywords = {astrometry, Galaxy: bulge, Galaxy: centre, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2004,
    month = mar,
   volume = 348,
    pages = {1439-1450},
      doi = {10.1111/j.1365-2966.2004.07457.x},
   adsurl = {http://adsabs.harvard.edu/abs/2004MNRAS.348.1439S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Annie12,
   author = {{Robin}, A.~C. and {Marshall}, D.~J. and {Schultheis}, M. and 
	{Reyl{\'e}}, C.},
    title = "{Stellar populations in the Milky Way bulge region: towards solving the Galactic bulge and bar shapes using 2MASS data}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.5744},
 keywords = {Galaxy: bulge, Galaxy: general, Galaxy: stellar content, Galaxy: structure, Galaxy: center, Galaxy: evolution},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A106},
    pages = {A106},
      doi = {10.1051/0004-6361/201116512},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...538A.106R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Misha16,
   author = {{Haywood}, M. and {Di Matteo}, P. and {Snaith}, O. and {Calamida}, A.
	},
    title = "{Hiding its age: the case for a younger bulge}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1606.04092},
 keywords = {Galaxy: abundances, Galaxy: disk, Galaxy: evolution, galaxies: evolution},
     year = 2016,
    month = sep,
   volume = 593,
      eid = {A82},
    pages = {A82},
      doi = {10.1051/0004-6361/201628816},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016A%26A...593A..82H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{GHB09,
   author = {{Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and {Bonifacio}, P.},
    title = "{A new implementation of the infrared flux method using the 2MASS catalogue}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0901.3034},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: stars, stars: abundances, stars: atmospheres, stars: fundamental parameters},
     year = 2009,
    month = apr,
   volume = 497,
    pages = {497-509},
      doi = {10.1051/0004-6361/200810904},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...497..497G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ELS62,
   author = {{Eggen}, O.~J. and {Lynden-Bell}, D. and {Sandage}, A.~R.},
    title = "{Evidence from the motions of old stars that the Galaxy collapsed.}",
  journal = {\apj},
     year = 1962,
    month = nov,
   volume = 136,
    pages = {748},
      doi = {10.1086/147433},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1962ApJ...136..748E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Immeli04,
   author = {{Immeli}, A. and {Samland}, M. and {Gerhard}, O. and {Westera}, P.
	},
    title = "{Gas physics, disk fragmentation,  and bulge formation in young galaxies}",
  journal = {\aap},
   eprint = {astro-ph/0312139},
 keywords = {ISM: kinematics and dynamics, ISM: structure, galaxies: abundances, galaxies: bulges, galaxies: evolution, galaxies: kinematics and dynamics},
     year = 2004,
    month = jan,
   volume = 413,
    pages = {547-561},
      doi = {10.1051/0004-6361:20034282},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004A%26A...413..547I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alvaro1,
   author = {{Rojas-Arriagada}, A. and {Recio-Blanco}, A. and {Hill}, V. and 
	{de Laverny}, P. and {Schultheis}, M. and {Babusiaux}, C. and 
	{Zoccali}, M. and {Minniti}, D. and {Gonzalez}, O.~A. and {Feltzing}, S. and 
	{Gilmore}, G. and {Randich}, S. and {Vallenari}, A. and {Alfaro}, E.~J. and 
	{Bensby}, T. and {Bragaglia}, A. and {Flaccomio}, E. and {Lanzafame}, A.~C. and 
	{Pancino}, E. and {Smiljanic}, R. and {Bergemann}, M. and {Costado}, M.~T. and 
	{Damiani}, F. and {Hourihane}, A. and {Jofr{\'e}}, P. and {Lardo}, C. and 
	{Magrini}, L. and {Maiorca}, E. and {Morbidelli}, L. and {Sbordone}, L. and 
	{Worley}, C.~C. and {Zaggia}, S. and {Wyse}, R.},
    title = "{The Gaia-ESO Survey: metallicity and kinematic trends in the Milky Way bulge}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1408.4558},
 keywords = {Galaxy: formation, Galaxy: abundances, Galaxy: bulge, Galaxy: stellar content, stars: abundances},
     year = 2014,
    month = sep,
   volume = 569,
      eid = {A103},
    pages = {A103},
      doi = {10.1051/0004-6361/201424121},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...569A.103R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{NessPop,
   author = {{Ness}, M. and {Freeman}, K. and {Athanassoula}, E. and {Wylie-de-Boer}, E. and 
	{Bland-Hawthorn}, J. and {Asplund}, M. and {Lewis}, G.~F. and 
	{Yong}, D. and {Lane}, R.~R. and {Kiss}, L.~L.},
    title = "{ARGOS - III. Stellar populations in the Galactic bulge of the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1212.1540},
 keywords = {stars: abundances, Galaxy: abundances, Galaxy: bulge, Galaxy: centre, Galaxy: evolution, Galaxy: formation},
     year = 2013,
    month = apr,
   volume = 430,
    pages = {836-857},
      doi = {10.1093/mnras/sts629},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.430..836N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ScannapiecoTissera03,
   author = {{Scannapieco}, C. and {Tissera}, P.~B.},
    title = "{The effects of mergers on the formation of disc-bulge systems in hierarchical clustering scenarios}",
  journal = {\mnras},
   eprint = {astro-ph/0208538},
 keywords = {methods: numerical, galaxies: evolution, galaxies: fundamental parameters, galaxies: interactions},
     year = 2003,
    month = feb,
   volume = 338,
    pages = {880-890},
      doi = {10.1046/j.1365-8711.2003.06133.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2003MNRAS.338..880S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McWilliamManu10,
   author = {{McWilliam}, A. and {Zoccali}, M.},
    title = "{Two Red Clumps and the X-shaped Milky Way Bulge}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1008.0519},
 keywords = {Galaxy: bulge, Galaxy: structure, stars: distances, stars: late-type},
     year = 2010,
    month = dec,
   volume = 724,
    pages = {1491-1502},
      doi = {10.1088/0004-637X/724/2/1491},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010ApJ...724.1491M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Alvaro2,
   author = {{Rojas-Arriagada}, A. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Mikolaitis}, {\v S}. and {Matteucci}, F. and {Spitoni}, E. and 
	{Schultheis}, M. and {Hayden}, M. and {Hill}, V. and {Zoccali}, M. and 
	{Minniti}, D. and {Gonzalez}, O.~A. and {Gilmore}, G. and {Randich}, S. and 
	{Feltzing}, S. and {Alfaro}, E.~J. and {Babusiaux}, C. and {Bensby}, T. and 
	{Bragaglia}, A. and {Flaccomio}, E. and {Koposov}, S.~E. and 
	{Pancino}, E. and {Bayo}, A. and {Carraro}, G. and {Casey}, A.~R. and 
	{Costado}, M.~T. and {Damiani}, F. and {Donati}, P. and {Franciosini}, E. and 
	{Hourihane}, A. and {Jofr{\'e}}, P. and {Lardo}, C. and {Lewis}, J. and 
	{Lind}, K. and {Magrini}, L. and {Morbidelli}, L. and {Sacco}, G.~G. and 
	{Worley}, C.~C. and {Zaggia}, S.},
    title = "{The Gaia-ESO Survey: Exploring the complex nature and origins of the Galactic bulge populations}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1704.03325},
 keywords = {Galaxy: bulge, Galaxy: formation, Galaxy: abundances, Galaxy: stellar content, stars: abundances},
     year = 2017,
    month = may,
   volume = 601,
      eid = {A140},
    pages = {A140},
      doi = {10.1051/0004-6361/201629160},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017A%26A...601A.140R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grieco12,
   author = {{Grieco}, V. and {Matteucci}, F. and {Pipino}, A. and {Cescutti}, G.
	},
    title = "{Chemical evolution of the Galactic bulge: different stellar populations and possible gradients}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1209.4462},
 keywords = {Galaxy: abundances, Galaxy: bulge, Galaxy: evolution},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A60},
    pages = {A60},
      doi = {10.1051/0004-6361/201219761},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...548A..60G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Van11,
   author = {{Hill}, V. and {Lecureur}, A. and {G{\'o}mez}, A. and {Zoccali}, M. and 
	{Schultheis}, M. and {Babusiaux}, C. and {Royer}, F. and {Barbuy}, B. and 
	{Arenou}, F. and {Minniti}, D. and {Ortolani}, S.},
    title = "{The metallicity distribution of bulge clump giants in Baade's window}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.5199},
 keywords = {Galaxy: bulge, Galaxy: formation, Galaxy: abundances, stars: abundances, stars: atmospheres},
     year = 2011,
    month = oct,
   volume = 534,
      eid = {A80},
    pages = {A80},
      doi = {10.1051/0004-6361/200913757},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...534A..80H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GES,
   author = {{Gilmore}, G. and {Randich}, S. and {Asplund}, M. and {Binney}, J. and 
	{Bonifacio}, P. and {Drew}, J. and {Feltzing}, S. and {Ferguson}, A. and 
	{Jeffries}, R. and {Micela}, G. and et al.},
    title = "{The Gaia-ESO Public Spectroscopic Survey}",
  journal = {The Messenger},
     year = 2012,
    month = mar,
   volume = 147,
    pages = {25-31},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012Msngr.147...25G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bensby13,
   author = {{Bensby}, T. and {Yee}, J.~C. and {Feltzing}, S. and {Johnson}, J.~A. and 
	{Gould}, A. and {Cohen}, J.~G. and {Asplund}, M. and {Mel{\'e}ndez}, J. and 
	{Lucatello}, S. and {Han}, C. and {Thompson}, I. and {Gal-Yam}, A. and 
	{Udalski}, A. and {Bennett}, D.~P. and {Bond}, I.~A. and {Kohei}, W. and 
	{Sumi}, T. and {Suzuki}, D. and {Suzuki}, K. and {Takino}, S. and 
	{Tristram}, P. and {Yamai}, N. and {Yonehara}, A.},
    title = "{Chemical evolution of the Galactic bulge as traced by microlensed dwarf and subgiant stars. V. Evidence for a wide age distribution and a complex MDF}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.6848},
 keywords = {gravitational lensing: micro, Galaxy: bulge, Galaxy:, formation, Galaxy: evolution, stars: abundances},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A147},
    pages = {A147},
      doi = {10.1051/0004-6361/201220678},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26A...549A.147B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DiMatteo15,
   author = {{Di Matteo}, P. and {G{\'o}mez}, A. and {Haywood}, M. and {Combes}, F. and 
	{Lehnert}, M.~D. and {Ness}, M. and {Snaith}, O.~N. and {Katz}, D. and 
	{Semelin}, B.},
    title = "{Why the Milky Way's bulge is not only a bar formed from a cold thin disk}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1411.1416},
 keywords = {methods: numerical, Galaxy: bulge, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: abundances},
     year = 2015,
    month = may,
   volume = 577,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201424457},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015A%26A...577A...1D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Oscar15,
   author = {{Gonzalez}, O.~A. and {Zoccali}, M. and {Vasquez}, S. and {Hill}, V. and 
	{Rejkuba}, M. and {Valenti}, E. and {Rojas-Arriagada}, A. and 
	{Renzini}, A. and {Babusiaux}, C. and {Minniti}, D. and {Brown}, T.~M.
	},
    title = "{The GIRAFFE Inner Bulge Survey (GIBS). II. Metallicity distributions and alpha element abundances at fixed Galactic latitude}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1508.02576},
 keywords = {Galaxy: bulge, Galaxy: abundances, Galaxy: formation, Galaxy: evolution},
     year = 2015,
    month = dec,
   volume = 584,
      eid = {A46},
    pages = {A46},
      doi = {10.1051/0004-6361/201526737},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015A%26A...584A..46G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schiavon16,
  author = {{Schiavon}, R.~P. and {Zamora}, O. and {Carrera}, R. and {Lucatello}, S. and 
	{Robin}, A.~C. and {Ness}, M. and {Martell}, S.~L. and {Smith}, V.~V. and 
	{Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and {Manchado}, A. and 
	{Sch{\"o}nrich}, R. and {Bastian}, N. and {Chiappini}, C. and 
	{Shetrone}, M. and {Mackereth}, J.~T. and {Williams}, R.~A. and 
	{M{\'e}sz{\'a}ros}, S. and {Allende Prieto}, C. and {Anders}, F. and 
	{Bizyaev}, D. and {Beers}, T.~C. and {Chojnowski}, S.~D. and 
	{Cunha}, K. and {Epstein}, C. and {Frinchaboy}, P.~M. and {Garc{\'{\i}}a P{\'e}rez}, A.~E. and 
	{Hearty}, F.~R. and {Holtzman}, J.~A. and {Johnson}, J.~A. and 
	{Kinemuchi}, K. and {Majewski}, S.~R. and {Muna}, D. and {Nidever}, D.~L. and 
	{Nguyen}, D.~C. and {O'Connell}, R.~W. and {Oravetz}, D. and 
	{Pan}, K. and {Pinsonneault}, M. and {Schneider}, D.~P. and 
	{Schultheis}, M. and {Simmons}, A. and {Skrutskie}, M.~F. and 
	{Sobeck}, J. and {Wilson}, J.~C. and {Zasowski}, G.},
    title = "{Chemical tagging with APOGEE: discovery of a large population of N-rich stars in the inner Galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1606.05651},
     year = 2017,
    month = feb,
   volume = 465,
    pages = {501-524},
      doi = {10.1093/mnras/stw2162},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017MNRAS.465..501S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2012A&A...548A.127M,
   author = {{Minchev}, I. and {Famaey}, B. and {Quillen}, A.~C. and {Dehnen}, W. and 
	{Martig}, M. and {Siebert}, A.},
    title = "{Radial migration does little for Galactic disc thickening}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1205.6475},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: evolution, galaxies: kinematics and dynamics},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A127},
    pages = {A127},
      doi = {10.1051/0004-6361/201219714},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...548A.127M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GrilleAMBRE,
   author = {{de Laverny}, P. and {Recio-Blanco}, A. and {Worley}, C.~C. and 
	{Plez}, B.},
    title = "{The AMBRE project: A new synthetic grid of high-resolution FGKM stellar spectra}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1205.2270},
 primaryClass = "astro-ph.SR",
 keywords = {stars: atmospheres, stars: fundamental parameters, stars: abundances, astronomical databases: miscellaneous, surveys},
     year = 2012,
    month = aug,
   volume = 544,
      eid = {A126},
    pages = {A126},
      doi = {10.1051/0004-6361/201219330},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...544A.126D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{KormendyKennicutt04,
   author = {{Kormendy}, J. and {Kennicutt}, Jr., R.~C.},
    title = "{Secular Evolution and the Formation of Pseudobulges in Disk Galaxies}",
  journal = {\araa},
   eprint = {astro-ph/0407343},
     year = 2004,
    month = sep,
   volume = 42,
    pages = {603-683},
      doi = {10.1146/annurev.astro.42.053102.134024},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004ARA%26A..42..603K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Prochaska2000,
   author = {{Prochaska}, J.~X. and {Naumov}, S.~O. and {Carney}, B.~W. and 
	{McWilliam}, A. and {Wolfe}, A.~M.},
    title = "{The Galactic Thick Disk Stellar Abundances}",
  journal = {\aj},
   eprint = {astro-ph/0008075},
 keywords = {Galaxy: Abundances, Galaxy: Formation, Stars: Abundances},
     year = 2000,
    month = nov,
   volume = 120,
    pages = {2513-2549},
      doi = {10.1086/316818},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2000AJ....120.2513P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Reid93,
   author = {{Reid}, M.~J.},
    title = "{The distance to the center of the Galaxy}",
  journal = {\araa},
 keywords = {Astrometry, Distance, Galactic Nuclei, Milky Way Galaxy, Astronomical Models, Globular Clusters, Water Masers},
     year = 1993,
   volume = 31,
    pages = {345-372},
      doi = {10.1146/annurev.aa.31.090193.002021},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1993ARA%26A..31..345R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MartinezValpuesta13,
   author = {{Martinez-Valpuesta}, I. and {Gerhard}, O.},
    title = "{Metallicity Gradients Through Disk Instability: A Simple Model for the Milky Way's Boxy Bulge}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1302.1613},
 keywords = {galaxies: evolution, Galaxy: abundances, Galaxy: bulge, Galaxy: kinematics and dynamics, Galaxy: structure, methods: numerical },
     year = 2013,
    month = mar,
   volume = 766,
      eid = {L3},
    pages = {L3},
      doi = {10.1088/2041-8205/766/1/L3},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...766L...3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{DiMatteo14,
   author = {{Di Matteo}, P. and {Haywood}, M. and {G{\'o}mez}, A. and {van Damme}, L. and 
	{Combes}, F. and {Hall{\'e}}, A. and {Semelin}, B. and {Lehnert}, M.~D. and 
	{Katz}, D.},
    title = "{Mapping a stellar disk into a boxy bulge: The outside-in part of the Milky Way bulge formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1404.0304},
 keywords = {methods: numerical, Galaxy: bulge, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: structure, galaxies: evolution},
     year = 2014,
    month = jul,
   volume = 567,
      eid = {A122},
    pages = {A122},
      doi = {10.1051/0004-6361/201322958},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...567A.122D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zwitter10,
   author = {{Zwitter}, T. and {Matijevi{\v c}}, G. and {Breddels}, M.~A. and 
	{Smith}, M.~C. and {Helmi}, A. and {Munari}, U. and {Bienaym{\'e}}, O. and 
	{Binney}, J. and {Bland-Hawthorn}, J. and {Boeche}, C. and {Brown}, A.~G.~A. and 
	{Campbell}, R. and {Freeman}, K.~C. and {Fulbright}, J. and 
	{Gibson}, B. and {Gilmore}, G. and {Grebel}, E.~K. and {Navarro}, J.~F. and 
	{Parker}, Q.~A. and {Seabroke}, G.~M. and {Siebert}, A. and 
	{Siviero}, A. and {Steinmetz}, M. and {Watson}, F.~G. and {Williams}, M. and 
	{Wyse}, R.~F.~G.},
    title = "{Distance determination for RAVE stars using stellar models . II. Most likely values assuming a standard stellar evolution scenario}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1007.4411},
 primaryClass = "astro-ph.SR",
 keywords = {stars: distances, catalogs, surveys, Galaxy: structure, Galaxy: stellar content, stars: statistics},
     year = 2010,
    month = nov,
   volume = 522,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/201014922},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...522A..54Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bird13,
   author = {{Bird}, J.~C. and {Kazantzidis}, S. and {Weinberg}, D.~H. and 
	{Guedes}, J. and {Callegari}, S. and {Mayer}, L. and {Madau}, P.
	},
    title = "{Inside out and Upside down: Tracing the Assembly of a Simulated Disk Galaxy Using Mono-age Stellar Populations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.0620},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: evolution, galaxies: spiral, Galaxy: evolution, Galaxy: formation, Galaxy: kinematics and dynamics, Galaxy: structure },
     year = 2013,
    month = aug,
   volume = 773,
      eid = {43},
    pages = {43},
      doi = {10.1088/0004-637X/773/1/43},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...773...43B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stinson13,
   author = {{Stinson}, G.~S. and {Bovy}, J. and {Rix}, H.-W. and {Brook}, C. and 
	{Ro{\v s}kar}, R. and {Dalcanton}, J.~J. and {Macci{\`o}}, A.~V. and 
	{Wadsley}, J. and {Couchman}, H.~M.~P. and {Quinn}, T.~R.},
    title = "{MaGICC thick disc - I. Comparing a simulated disc formed with stellar feedback to the Milky Way}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1301.5318},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, galaxies: formation, galaxies: structure},
     year = 2013,
    month = nov,
   volume = 436,
    pages = {625-634},
      doi = {10.1093/mnras/stt1600},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.436..625S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bilir12,
   author = {{Bilir}, S. and {Karaali}, S. and {Ak}, S. and {{\"O}nal}, {\"O}. and 
	{Da{\v g}tekin}, N.~D. and {Yontan}, T. and {Gilmore}, G. and 
	{Seabroke}, G.~M.},
    title = "{Local stellar kinematics from RAVE data - III. Radial and vertical metallicity gradients based on red clump stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.3065},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, Galaxy: abundances, Galaxy: disc, Galaxy: evolution},
     year = 2012,
    month = apr,
   volume = 421,
    pages = {3362-3374},
      doi = {10.1111/j.1365-2966.2012.20561.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.421.3362B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kordo13MWTD,
   author = {{Kordopatis}, G. and {Gilmore}, G. and {Wyse}, R.~F.~G. and 
	{Steinmetz}, M. and {Siebert}, A. and {Bienaym{\'e}}, O. and 
	{McMillan}, P.~J. and {Minchev}, I. and {Zwitter}, T. and {Gibson}, B.~K. and 
	{Seabroke}, G. and {Grebel}, E.~K. and {Bland-Hawthorn}, J. and 
	{Boeche}, C. and {Freeman}, K.~C. and {Munari}, U. and {Navarro}, J.~F. and 
	{Parker}, Q. and {Reid}, W.~A. and {Siviero}, A.},
    title = "{In the thick of it: metal-poor disc stars in RAVE}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.1919},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: disc, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure},
     year = 2013,
    month = dec,
   volume = 436,
    pages = {3231-3246},
      doi = {10.1093/mnras/stt1804},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013MNRAS.436.3231K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schlegelMapas,
   author = {{Schlegel}, D.~J. and {Finkbeiner}, D.~P. and {Davis}, M.},
    title = "{Maps of Dust Infrared Emission for Use in Estimation of Reddening and Cosmic Microwave Background Radiation Foregrounds}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9710327},
 keywords = {COSMOLOGY: DIFFUSE RADIATION, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, ISM: DUST, EXTINCTION, INTERPLANETARY MEDIUM, INFRARED: ISM: CONTINUUM},
     year = 1998,
    month = jun,
   volume = 500,
    pages = {525},
      doi = {10.1086/305772},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500..525S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Loebman,
   author = {{Loebman}, S.~R. and {Ro{\v s}kar}, R. and {Debattista}, V.~P. and 
	{Ivezi{\'c}}, {\v Z}. and {Quinn}, T.~R. and {Wadsley}, J.},
    title = "{The Genesis of the Milky Way's Thick Disk Via Stellar Migration}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1009.5997},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: spiral, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure, solar neighborhood},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {8},
    pages = {8},
      doi = {10.1088/0004-637X/737/1/8},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011ApJ...737....8L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Minchev10,
   author = {{Minchev}, I. and {Famaey}, B.},
    title = "{A New Mechanism for Radial Migration in Galactic Disks: Spiral-Bar Resonance Overlap}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0911.1794},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: abundances, galaxies: evolution, galaxies: kinematics and dynamics, galaxies: spiral, solar neighborhood},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {112-121},
      doi = {10.1088/0004-637X/722/1/112},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010ApJ...722..112M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bournaud,
   author = {{Bournaud}, F. and {Elmegreen}, B.~G. and {Martig}, M.},
    title = "{The Thick Disks of Spiral Galaxies as Relics from Gas-rich, Turbulent, Clumpy Disks at High Redshift}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0910.3677},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: formation, galaxies: high-redshift, Galaxy: disk, ISM: structure},
     year = 2009,
    month = dec,
   volume = 707,
    pages = {L1-L5},
      doi = {10.1088/0004-637X/707/1/L1},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009ApJ...707L...1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Brook1,
   author = {{Brook}, C.~B. and {Kawata}, D. and {Gibson}, B.~K. and {Freeman}, K.~C.
	},
    title = "{The Emergence of the Thick Disk in a Cold Dark Matter Universe}",
  journal = {\apj},
   eprint = {astro-ph/0405306},
 keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxy: Disk},
     year = 2004,
    month = sep,
   volume = 612,
    pages = {894-899},
      doi = {10.1086/422709},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004ApJ...612..894B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Brook2,
   author = {{Brook}, C. and {Richard}, S. and {Kawata}, D. and {Martel}, H. and 
	{Gibson}, B.~K.},
    title = "{Two Disk Components from a Gas-Rich Disk-Disk Merger}",
  journal = {\apj},
   eprint = {astro-ph/0611748},
 keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: Interactions, Galaxies: Structure},
     year = 2007,
    month = mar,
   volume = 658,
    pages = {60-64},
      doi = {10.1086/511056},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...658...60B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Jones83,
   author = {{Jones}, B.~J.~T. and {Wyse}, R.~F.~G.},
    title = "{The formation of disc galaxies}",
  journal = {\aap},
 keywords = {Astronomical Models, Cosmology, Disk Galaxies, Galactic Evolution, Compton Effect, Density Distribution, Galactic Bulge, Gravitational Collapse, Stellar Evolution},
     year = 1983,
    month = apr,
   volume = 120,
    pages = {165-180},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1983A%26A...120..165J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Villalobos,
   author = {{Villalobos}, {\'A}. and {Helmi}, A.},
    title = "{Simulations of minor mergers - I. General properties of thick discs}",
  journal = {\mnras},
 keywords = {Galaxy: disc , Galaxy: formation , Galaxy: kinematics and dynamics , galaxies: formation , galaxies: kinematics and dynamics , galaxies: structure},
     year = 2008,
    month = dec,
   volume = 391,
    pages = {1806-1827},
      doi = {10.1111/j.1365-2966.2008.13979.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.391.1806V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Quinn,
   author = {{Quinn}, P.~J. and {Hernquist}, L. and {Fullagar}, D.~P.},
    title = "{Heating of galactic disks by mergers}",
  journal = {\apj},
 keywords = {Computational Astrophysics, Galactic Evolution, Galactic Structure, Interacting Galaxies, Spiral Galaxies, Abundance, Accretion Disks, Galactic Halos, Many Body Problem},
     year = 1993,
    month = jan,
   volume = 403,
    pages = {74-93},
      doi = {10.1086/172184},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1993ApJ...403...74Q},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Abadi,
   author = {{Abadi}, M.~G. and {Navarro}, J.~F. and {Steinmetz}, M. and 
	{Eke}, V.~R.},
    title = "{Simulations of Galaxy Formation in a {$\Lambda$} Cold Dark Matter Universe. II. The Fine Structure of Simulated Galactic Disks}",
  journal = {\apj},
   eprint = {astro-ph/0212282},
 keywords = {Cosmology: Dark Matter, Galaxies: Evolution, Galaxies: Formation, Galaxies: Structure, Methods: Numerical},
     year = 2003,
    month = nov,
   volume = 597,
    pages = {21-34},
      doi = {10.1086/378316},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2003ApJ...597...21A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Statler,
   author = {{Statler}, T.~S.},
    title = "{Orbital decay in aspherical galaxies. I - Oblate systems}",
  journal = {\apj},
 keywords = {Galactic Structure, Oblate Spheroids, Orbit Decay, Star Distribution, Stellar Motions, Stellar Orbits, Asphericity, Circular Orbits, Decay Rates, Star Formation},
     year = 1988,
    month = aug,
   volume = 331,
    pages = {71-101},
      doi = {10.1086/166539},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1988ApJ...331...71S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Norris99,
   author = {{Norris}, J.~E.},
    title = "{The Galactic Thick Disk - Status}",
  journal = {\apss},
     year = 1999,
    month = jul,
   volume = 265,
    pages = {213-220},
      doi = {10.1023/A:1002180131034},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999Ap%26SS.265..213N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{GilmoreReid,
   author = {{Gilmore}, G. and {Reid}, N.},
    title = "{New light on faint stars. III - Galactic structure towards the South Pole and the Galactic thick disc}",
  journal = {\mnras},
 keywords = {Galactic Structure, Southern Sky, Stellar Luminosity, Stellar Mass, Stellar Structure, Astronomical Photometry, Density Distribution, Metallicity, Star Distribution},
     year = 1983,
    month = mar,
   volume = 202,
    pages = {1025-1047},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1983MNRAS.202.1025G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Yoshii,
   author = {{Yoshii}, Y.},
    title = "{Density Distribution of Faint Stars in the Direction of the North Galactic Pole}",
  journal = {\pasj},
     year = 1982,
   volume = 34,
    pages = {365},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1982PASJ...34..365Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bovy12Mono,
   author = {{Bovy}, J. and {Rix}, H.-W. and {Liu}, C. and {Hogg}, D.~W. and 
	{Beers}, T.~C. and {Lee}, Y.~S.},
    title = "{The Spatial Structure of Mono-abundance Sub-populations of the Milky Way Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.1724},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: disk, Galaxy: evolution, Galaxy: formation, Galaxy: fundamental parameters, Galaxy: structure},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {148},
    pages = {148},
      doi = {10.1088/0004-637X/753/2/148},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...753..148B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{RAVEDr1,
   author = {{Steinmetz}, M. and {Zwitter}, T. and {Siebert}, A. and {Watson}, F.~G. and 
	{Freeman}, K.~C. and {Munari}, U. and {Campbell}, R. and {Williams}, M. and 
	{Seabroke}, G.~M. and {Wyse}, R.~F.~G. and {Parker}, Q.~A. and 
	{Bienaym{\'e}}, O. and {Roeser}, S. and {Gibson}, B.~K. and 
	{Gilmore}, G. and {Grebel}, E.~K. and {Helmi}, A. and {Navarro}, J.~F. and 
	{Burton}, D. and {Cass}, C.~J.~P. and {Dawe}, J.~A. and {Fiegert}, K. and 
	{Hartley}, M. and {Russell}, K.~S. and {Saunders}, W. and {Enke}, H. and 
	{Bailin}, J. and {Binney}, J. and {Bland-Hawthorn}, J. and {Boeche}, C. and 
	{Dehnen}, W. and {Eisenstein}, D.~J. and {Evans}, N.~W. and 
	{Fiorucci}, M. and {Fulbright}, J.~P. and {Gerhard}, O. and 
	{Jauregi}, U. and {Kelz}, A. and {Mijovi{\'c}}, L. and {Minchev}, I. and 
	{Parmentier}, G. and {Pe{\~n}arrubia}, J. and {Quillen}, A.~C. and 
	{Read}, M.~A. and {Ruchti}, G. and {Scholz}, R.-D. and {Siviero}, A. and 
	{Smith}, M.~C. and {Sordo}, R. and {Veltz}, L. and {Vidrih}, S. and 
	{von Berlepsch}, R. and {Boyle}, B.~J. and {Schilbach}, E.},
    title = "{The Radial Velocity Experiment (RAVE): First Data Release}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0606211},
 keywords = {Catalogs, Stars: Fundamental Parameters, Surveys},
     year = 2006,
    month = oct,
   volume = 132,
    pages = {1645-1668},
      doi = {10.1086/506564},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006AJ....132.1645S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GCS,
   author = {{Nordstr{\"o}m}, B. and {Mayor}, M. and {Andersen}, J. and {Holmberg}, J. and 
	{Pont}, F. and {J{\o}rgensen}, B.~R. and {Olsen}, E.~H. and 
	{Udry}, S. and {Mowlavi}, N.},
    title = "{The Geneva-Copenhagen survey of the Solar neighbourhood. Ages, metallicities, and kinematic properties of {\tilde}14 000 F and G dwarfs}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0405198},
 keywords = {Galaxy: disk, Galaxy: solar neighbourhood, Galaxy: stellar content, Galaxy: kinematics and dynamics, Galaxy: evolution, stars: fundamental parameters},
     year = 2004,
    month = may,
   volume = 418,
    pages = {989-1019},
      doi = {10.1051/0004-6361:20035959},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004A%26A...418..989N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Segue1,
   author = {{Yanny}, B. and {Rockosi}, C. and {Newberg}, H.~J. and {Knapp}, G.~R. and 
	{Adelman-McCarthy}, J.~K. and {Alcorn}, B. and {Allam}, S. and 
	{Allende Prieto}, C. and {An}, D. and {Anderson}, K.~S.~J. and 
	{Anderson}, S. and {Bailer-Jones}, C.~A.~L. and {Bastian}, S. and 
	{Beers}, T.~C. and {Bell}, E. and {Belokurov}, V. and {Bizyaev}, D. and 
	{Blythe}, N. and {Bochanski}, J.~J. and {Boroski}, W.~N. and 
	{Brinchmann}, J. and {Brinkmann}, J. and {Brewington}, H. and 
	{Carey}, L. and {Cudworth}, K.~M. and {Evans}, M. and {Evans}, N.~W. and 
	{Gates}, E. and {G{\"a}nsicke}, B.~T. and {Gillespie}, B. and 
	{Gilmore}, G. and {Nebot Gomez-Moran}, A. and {Grebel}, E.~K. and 
	{Greenwell}, J. and {Gunn}, J.~E. and {Jordan}, C. and {Jordan}, W. and 
	{Harding}, P. and {Harris}, H. and {Hendry}, J.~S. and {Holder}, D. and 
	{Ivans}, I.~I. and {Ivezi{\v c}}, {\v Z}. and {Jester}, S. and 
	{Johnson}, J.~A. and {Kent}, S.~M. and {Kleinman}, S. and {Kniazev}, A. and 
	{Krzesinski}, J. and {Kron}, R. and {Kuropatkin}, N. and {Lebedeva}, S. and 
	{Lee}, Y.~S. and {French Leger}, R. and {L{\'e}pine}, S. and 
	{Levine}, S. and {Lin}, H. and {Long}, D.~C. and {Loomis}, C. and 
	{Lupton}, R. and {Malanushenko}, O. and {Malanushenko}, V. and 
	{Margon}, B. and {Martinez-Delgado}, D. and {McGehee}, P. and 
	{Monet}, D. and {Morrison}, H.~L. and {Munn}, J.~A. and {Neilsen}, Jr., E.~H. and 
	{Nitta}, A. and {Norris}, J.~E. and {Oravetz}, D. and {Owen}, R. and 
	{Padmanabhan}, N. and {Pan}, K. and {Peterson}, R.~S. and {Pier}, J.~R. and 
	{Platson}, J. and {Re Fiorentin}, P. and {Richards}, G.~T. and 
	{Rix}, H.-W. and {Schlegel}, D.~J. and {Schneider}, D.~P. and 
	{Schreiber}, M.~R. and {Schwope}, A. and {Sibley}, V. and {Simmons}, A. and 
	{Snedden}, S.~A. and {Allyn Smith}, J. and {Stark}, L. and {Stauffer}, F. and 
	{Steinmetz}, M. and {Stoughton}, C. and {SubbaRao}, M. and {Szalay}, A. and 
	{Szkody}, P. and {Thakar}, A.~R. and {Sivarani}, T. and {Tucker}, D. and 
	{Uomoto}, A. and {Vanden Berk}, D. and {Vidrih}, S. and {Wadadekar}, Y. and 
	{Watters}, S. and {Wilhelm}, R. and {Wyse}, R.~F.~G. and {Yarger}, J. and 
	{Zucker}, D.},
    title = "{SEGUE: A Spectroscopic Survey of 240,000 Stars with g = 14-20}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0902.1781},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, Galaxy: stellar content, Galaxy: structure, stars: abundances, stars: fundamental parameters, stars: general},
     year = 2009,
    month = may,
   volume = 137,
      eid = {4377},
    pages = {4377-4399},
      doi = {10.1088/0004-6256/137/5/4377},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009AJ....137.4377Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Segue2,
   author = {{Eisenstein}, D.~J. and {Weinberg}, D.~H. and {Agol}, E. and 
	{Aihara}, H. and {Allende Prieto}, C. and {Anderson}, S.~F. and 
	{Arns}, J.~A. and {Aubourg}, {\'E}. and {Bailey}, S. and {Balbinot}, E. and et al.},
    title = "{SDSS-III: Massive Spectroscopic Surveys of the Distant Universe, the Milky Way, and Extra-Solar Planetary Systems}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1101.1529},
 primaryClass = "astro-ph.IM",
 keywords = {cosmology: observations, Galaxy: evolution, planets and satellites: detection, surveys},
     year = 2011,
    month = sep,
   volume = 142,
      eid = {72},
    pages = {72},
      doi = {10.1088/0004-6256/142/3/72},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011AJ....142...72E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lee2011b,
   author = {{Lee}, Y.~S. and {Beers}, T.~C. and {An}, D. and {Ivezi{\'c}}, {\v Z}. and 
	{Just}, A. and {Rockosi}, C.~M. and {Morrison}, H.~L. and {Johnson}, J.~A. and 
	{Sch{\"o}nrich}, R. and {Bird}, J. and {Yanny}, B. and {Harding}, P. and 
	{Rocha-Pinto}, H.~J.},
    title = "{Formation and Evolution of the Disk System of the Milky Way: [{$\alpha$}/Fe] Ratios and Kinematics of the SEGUE G-dwarf Sample}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.3114},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, Galaxy: formation, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2011,
    month = sep,
   volume = 738,
      eid = {187},
    pages = {187},
      doi = {10.1088/0004-637X/738/2/187},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011ApJ...738..187L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Smolinski2011,
   author = {{Smolinski}, J.~P. and {Lee}, Y.~S. and {Beers}, T.~C. and {An}, D. and 
	{Bickerton}, S.~J. and {Johnson}, J.~A. and {Loomis}, C.~P. and 
	{Rockosi}, C.~M. and {Sivarani}, T. and {Yanny}, B.},
    title = "{The SEGUE Stellar Parameter Pipeline. IV. Validation with an Extended Sample of Galactic Globular and Open Clusters}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1008.1959},
 primaryClass = "astro-ph.GA",
 keywords = {methods: data analysis, stars: abundances, stars: fundamental parameters, surveys, techniques: spectroscopic},
     year = 2011,
    month = mar,
   volume = 141,
      eid = {89},
    pages = {89},
      doi = {10.1088/0004-6256/141/3/89},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011AJ....141...89S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lee2011a,
   author = {{Lee}, Y.~S. and {Beers}, T.~C. and {Allende Prieto}, C. and 
	{Lai}, D.~K. and {Rockosi}, C.~M. and {Morrison}, H.~L. and 
	{Johnson}, J.~A. and {An}, D. and {Sivarani}, T. and {Yanny}, B.
	},
    title = "{The SEGUE Stellar Parameter Pipeline. V. Estimation of Alpha-element Abundance Ratios from Low-resolution SDSS/SEGUE Stellar Spectra}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1010.2934},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, stars: abundances, stars: fundamental parameters, surveys, techniques: imaging spectroscopy},
     year = 2011,
    month = mar,
   volume = 141,
      eid = {90},
    pages = {90},
      doi = {10.1088/0004-6256/141/3/90},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011AJ....141...90L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CasettiDinescu2011,
   author = {{Casetti-Dinescu}, D.~I. and {Girard}, T.~M. and {Korchagin}, V.~I. and 
	{van Altena}, W.~F.},
    title = "{The Three-dimensional Velocity Structure of the Thick Disk from SPM4 and RAVE DR2}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1011.6253},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2011,
    month = feb,
   volume = 728,
      eid = {7},
    pages = {7},
      doi = {10.1088/0004-637X/728/1/7},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011ApJ...728....7C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Juric2008,
   author = {{Juri{\'c}}, M. and {Ivezi{\'c}}, {\v Z}. and {Brooks}, A. and 
	{Lupton}, R.~H. and {Schlegel}, D. and {Finkbeiner}, D. and 
	{Padmanabhan}, N. and {Bond}, N. and {Sesar}, B. and {Rockosi}, C.~M. and 
	{Knapp}, G.~R. and {Gunn}, J.~E. and {Sumi}, T. and {Schneider}, D.~P. and 
	{Barentine}, J.~C. and {Brewington}, H.~J. and {Brinkmann}, J. and 
	{Fukugita}, M. and {Harvanek}, M. and {Kleinman}, S.~J. and 
	{Krzesinski}, J. and {Long}, D. and {Neilsen}, Jr., E.~H. and 
	{Nitta}, A. and {Snedden}, S.~A. and {York}, D.~G.},
    title = "{The Milky Way Tomography with SDSS. I. Stellar Number Density Distribution}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0510520},
 keywords = {Galaxy: Disk, Galaxy: Fundamental Parameters, Galaxy: Halo, Galaxy: Structure},
     year = 2008,
    month = feb,
   volume = 673,
    pages = {864-914},
      doi = {10.1086/523619},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...673..864J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ChivaBeers,
   author = {{Chiba}, M. and {Beers}, T.~C.},
    title = "{Kinematics of Metal-poor Stars in the Galaxy. III. Formation of the Stellar Halo and Thick Disk as Revealed from a Large Sample of Nonkinematically Selected Stars}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0003087},
 keywords = {Galaxy: Abundances, Galaxy: Evolution, Galaxy: Halo, Stars: Population II},
     year = 2000,
    month = jun,
   volume = 119,
    pages = {2843-2865},
      doi = {10.1086/301409},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2000AJ....119.2843C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{WyseGilmore95,
   author = {{Wyse}, R.~F.~G. and {Gilmore}, G.},
    title = "{Chemistry and Kinematics in the Solar Neighborhood: Implications for Stellar Populations and for Galaxy Evolution}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/9509007},
 keywords = {SOLAR NEIGHBORHOOD, GALAXY: EVOLUTION, STARS: ABUNDANCES},
     year = 1995,
    month = dec,
   volume = 110,
    pages = {2771},
      doi = {10.1086/117729},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1995AJ....110.2771W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Fuhrmann08,
   author = {{Fuhrmann}, K.},
    title = "{Nearby stars of the Galactic disc and halo - IV}",
  journal = {\mnras},
 keywords = {stars: fundamental parameters , Galaxy: evolution , Galaxy: formation , Galaxy: stellar content},
     year = 2008,
    month = feb,
   volume = 384,
    pages = {173-224},
      doi = {10.1111/j.1365-2966.2007.12671.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.384..173F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bensby05,
   author = {{Bensby}, T. and {Feltzing}, S. and {Lundstr{\"o}m}, I. and 
	{Ilyin}, I.},
    title = "{{$\alpha$}-, r-, and s-process element trends in the Galactic thin and thick disks}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0412132},
 keywords = {, stars: fundamental parameters, stars: abundances, Galaxy:, disk, Galaxy: formation, Galaxy: abundances, Galaxy:, kinematics and dynamics},
     year = 2005,
    month = apr,
   volume = 433,
    pages = {185-203},
      doi = {10.1051/0004-6361:20040332},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005A%26A...433..185B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bensby07,
   author = {{Bensby}, T. and {Zenn}, A.~R. and {Oey}, M.~S. and {Feltzing}, S.
	},
    title = "{Tracing the Galactic Thick Disk to Solar Metallicities}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0705.2060},
 keywords = {Galaxy: Disk, Galaxy: Evolution, Galaxy: Formation, Galaxy: Solar Neighborhood, Stars: Abundances, Stars: Kinematics},
     year = 2007,
    month = jul,
   volume = 663,
    pages = {L13-L16},
      doi = {10.1086/519792},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007ApJ...663L..13B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{FreemanBH,
   author = {{Freeman}, K. and {Bland-Hawthorn}, J.},
    title = "{The New Galaxy: Signatures of Its Formation}",
  journal = {\araa},
   eprint = {arXiv:astro-ph/0208106},
 keywords = {osmology, local group, stellar populations, stellar kinematics},
     year = 2002,
   volume = 40,
    pages = {487-537},
      doi = {10.1146/annurev.astro.40.060401.093840},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002ARA%26A..40..487F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schiavon16b,
   author = {{Schiavon}, R.~P. and {Johnson}, J.~A. and {Frinchaboy}, P.~M. and 
	{Zasowski}, G. and {M{\'e}sz{\'a}ros}, S. and {Garc{\'{\i}}a-Hern{\'a}ndez}, D.~A. and 
	{Cohen}, R.~E. and {Tang}, B. and {Villanova}, S. and {Geisler}, D. and 
	{Beers}, T.~C. and {Fern{\'a}ndez-Trincado}, J.~G. and {Garc{\'{\i}}a P{\'e}rez}, A.~E. and 
	{Lucatello}, S. and {Majewski}, S.~R. and {Martell}, S.~L. and 
	{O'Connell}, R.~W. and {Prieto}, C.~A. and {Bizyaev}, D. and 
	{Carrera}, R. and {Lane}, R.~R. and {Malanushenko}, E. and {Malanushenko}, V. and 
	{Mu{\~n}oz}, R.~R. and {Nitschelm}, C. and {Oravetz}, D. and 
	{Pan}, K. and {Roman-Lopes}, A. and {Schultheis}, M. and {Simmons}, A.
	},
    title = "{APOGEE chemical abundances of globular cluster giants in the inner Galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1611.03086},
 keywords = {stars: abundances, Galaxy: bulge, globular clusters: general},
     year = 2017,
    month = apr,
   volume = 466,
    pages = {1010-1018},
      doi = {10.1093/mnras/stw3093},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017MNRAS.466.1010S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

   
@ARTICLE{RixBovy,
   author = {{Rix}, H.-W. and {Bovy}, J.},
    title = "{The Milky Way's stellar disk. Mapping and modeling the Galactic disk}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1301.3168},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: Disk, dynamics and kinematics, formation and evolution, stellar populations, Surveys},
     year = 2013,
    month = may,
   volume = 21,
    pages = {61},
      doi = {10.1007/s00159-013-0061-8},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26ARv..21...61R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu,
   author = {{Liu}, C. and {van de Ven}, G.},
    title = "{Chemo-orbital evidence from SDSS/SEGUE G-type dwarf stars for a mixed origin of the Milky Way's thick disc}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1201.1635},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: disc, Galaxy: formation, Galaxy: kinematics and dynamics },
     year = 2012,
    month = sep,
   volume = 425,
    pages = {2144-2156},
      doi = {10.1111/j.1365-2966.2012.21551.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.425.2144L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bovy2012a,
   author = {{Bovy}, J. and {Rix}, H.-W. and {Hogg}, D.~W.},
    title = "{The Milky Way Has No Distinct Thick Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.6585},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: disk, Galaxy: evolution, Galaxy: formation, Galaxy: fundamental parameters, Galaxy: structure},
     year = 2012,
    month = jun,
   volume = 751,
      eid = {131},
    pages = {131},
      doi = {10.1088/0004-637X/751/2/131},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...751..131B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schlesinger,
   author = {{Schlesinger}, K.~J. and {Johnson}, J.~A. and {Rockosi}, C.~M. and 
	{Lee}, Y.~S. and {Morrison}, H.~L. and {Sch{\"o}nrich}, R. and 
	{Allende Prieto}, C. and {Beers}, T.~C. and {Yanny}, B. and 
	{Harding}, P. and {Schneider}, D.~P. and {Chiappini}, C. and 
	{da Costa}, L.~N. and {Maia}, M.~A.~G. and {Minchev}, I. and 
	{Rocha-Pinto}, H. and {Santiago}, B.~X.},
    title = "{The Metallicity Distribution Functions of SEGUE G and K Dwarfs: Constraints for Disk Chemical Evolution and Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.2214},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: disk, Galaxy: evolution, Galaxy: stellar content, Galaxy: structure, stars: abundances, surveys },
     year = 2012,
    month = dec,
   volume = 761,
      eid = {160},
    pages = {160},
      doi = {10.1088/0004-637X/761/2/160},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...761..160S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Adibekyan2013,
   author = {{Adibekyan}, V.~Z. and {Figueira}, P. and {Santos}, N.~C. and 
	{Hakobyan}, A.~A. and {Sousa}, S.~G. and {Pace}, G. and {Delgado Mena}, E. and 
	{Robin}, A.~C. and {Israelian}, G. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I.
	},
    title = "{Kinematics and chemical properties of the Galactic stellar populations. The HARPS FGK dwarfs sample}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1304.2561},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, stars: kinematics and dynamics, Galaxy: disk},
     year = 2013,
    month = jun,
   volume = 554,
      eid = {A44},
    pages = {A44},
      doi = {10.1051/0004-6361/201321520},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26A...554A..44A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Adibekyan2012,
   author = {{Adibekyan}, V.~Z. and {Sousa}, S.~G. and {Santos}, N.~C. and 
	{Delgado Mena}, E. and {Gonz{\'a}lez Hern{\'a}ndez}, J.~I. and 
	{Israelian}, G. and {Mayor}, M. and {Khachatryan}, G.},
    title = "{Chemical abundances of 1111 FGK stars from the HARPS GTO planet search program. Galactic stellar populations and planets}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1207.2388},
 primaryClass = "astro-ph.EP",
 keywords = {stars: abundances, planetary systems, stars: fundamental parameters, Galaxy: disk, solar neighborhood, stars: kinematics and dynamics},
     year = 2012,
    month = sep,
   volume = 545,
      eid = {A32},
    pages = {A32},
      doi = {10.1051/0004-6361/201219401},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...545A..32A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haywood2013,
   author = {{Haywood}, M. and {Di Matteo}, P. and {Lehnert}, M. and {Katz}, D. and 
	{Gomez}, A.},
    title = "{The age structure of stellar populations in the solar vicinity. Clues of a two-phase formation history of the Milky Way disk}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1305.4663},
 primaryClass = "astro-ph.GA",
 keywords = {Astrophysics - Galaxy Astrophysics},
     year = 2013,
    month = may,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013arXiv1305.4663H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ramirez,
   author = {{Ram{\'{\i}}rez}, I. and {Allende Prieto}, C. and {Lambert}, D.~L.
	},
    title = "{Oxygen Abundances in Nearby FGK Stars and the Galactic Chemical Evolution of the Local Disk and Halo}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.1582},
 primaryClass = "astro-ph.SR",
 keywords = {Galaxy: disk, Galaxy: evolution, Galaxy: formation, stars: abundances, stars: atmospheres, stars: fundamental parameters },
     year = 2013,
    month = feb,
   volume = 764,
      eid = {78},
    pages = {78},
      doi = {10.1088/0004-637X/764/1/78},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...764...78R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{GESMessenger,
   author = {{Gilmore}, G. and {Randich}, S. and {Asplund}, M. and {Binney}, J. and 
	{Bonifacio}, P. and {Drew}, J. and {Feltzing}, S. and {Ferguson}, A. and 
	{Jeffries}, R. and {Micela}, G. and {Negueruela}, I. and {Prusti}, T. and 
	{Rix}, H.-W. and {Vallenari}, A. and {Alfaro}, E. and {Allende-Prieto}, C. and 
	{Babusiaux}, C. and {Bensby}, T. and {Blomme}, R. and {Bragaglia}, A. and 
	{Flaccomio}, E. and {Fran{\c c}ois}, P. and {Irwin}, M. and 
	{Koposov}, S. and {Korn}, A. and {Lanzafame}, A. and {Pancino}, E. and 
	{Paunzen}, E. and {Recio-Blanco}, A. and {Sacco}, G. and {Smiljanic}, R. and 
	{Van Eck}, S. and {Walton}, N.},
    title = "{The Gaia-ESO Public Spectroscopic Survey}",
  journal = {The Messenger},
     year = 2012,
    month = mar,
   volume = 147,
    pages = {25-31},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012Msngr.147...25G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DR1,
   author = {{Gilmore}, G. and {Randich}, S. and et al.},
    title = "{The Gaia-ESO Public Spectroscopic Survey Data Release 1}",
  journal = {\aap},
     year = 2014
}

@ARTICLE{GESVrad,
   author = {{Koposov}, S. et al.},
    title = "{The Gaia-ESO Public Spectroscopic Survey radial velocity pipeline}",
  journal = {\aap},
     year = 2014
}

@ARTICLE{WP10DR1,
   author = {{Recio-Blanco}, A. and {Allende Prieto}, C. and et al.},
    title = "{The Gaia-ESO Public Spectroscopic Survey DR1: analysis of GIRAFFE spectra of FGK-type stars}",
  journal = {\aap},
     year = 2014
}

@ARTICLE{Sarunas,
   author = {{Mikolaitis}, A. and {Recio-Blanco}, A. and {et al.}},
    title = "{Individual element abundances in the GES DR1 field disc stars data}",
  journal = {\aap},
     year = 2014
}

@ARTICLE{Matisse,
   author = {{Recio-Blanco}, A. and {Bijaoui}, A. and {de Laverny}, P.},
    title = "{Automated derivation of stellar atmospheric parameters and chemical abundances: the MATISSE algorithm}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0604385},
 keywords = {methods: data analysis: techniques: spectroscopic: stars: abundances: stars: fundamental parameters: Galaxy: stellar content, methods: data analysis, techniques: spectroscopic, stars: abundances, stars: fundamental parameters, Galaxy: stellar content},
     year = 2006,
    month = jul,
   volume = 370,
    pages = {141-150},
      doi = {10.1111/j.1365-2966.2006.10455.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006MNRAS.370..141R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferre,
   author = {{Allende Prieto}, C. and {Beers}, T.~C. and {Wilhelm}, R. and 
	{Newberg}, H.~J. and {Rockosi}, C.~M. and {Yanny}, B. and {Lee}, Y.~S.
	},
    title = "{A Spectroscopic Study of the Ancient Milky Way: F- and G-Type Stars in the Third Data Release of the Sloan Digital Sky Survey}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0509812},
 keywords = {Galaxy: Stellar Content, Galaxy: Structure, Stars: Abundances, Stars: Fundamental Parameters},
     year = 2006,
    month = jan,
   volume = 636,
    pages = {804-820},
      doi = {10.1086/498131},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...636..804A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{SME,
   author = {{Valenti}, J.~A. and {Piskunov}, N.},
    title = "{Spectroscopy made easy: A new tool for fitting observations with synthetic spectra.}",
  journal = {\aaps},
 keywords = {RADIATIVE TRANSFER, METHODS: NUMERICAL, TECHNIQUES: SPECTROSCOPIC, STARS: FUNDAMENTAL PARAMETERS, SUN: FUNDAMENTAL PARAMETERS, ATOMIC DATA},
     year = 1996,
    month = sep,
   volume = 118,
    pages = {595-603},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1996A%26AS..118..595V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ppmxl,
   author = {{Roeser}, S. and {Demleitner}, M. and {Schilbach}, E.},
    title = "{The PPMXL Catalog of Positions and Proper Motions on the ICRS. Combining USNO-B1.0 and the Two Micron All Sky Survey (2MASS)}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1003.5852},
 primaryClass = "astro-ph.GA",
 keywords = {astrometry, catalogs, Galaxy: kinematics and dynamics, proper motions},
     year = 2010,
    month = jun,
   volume = 139,
    pages = {2440-2447},
      doi = {10.1088/0004-6256/139/6/2440},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010AJ....139.2440R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bonifacio00,
   author = {{Bonifacio}, P. and {Monai}, S. and {Beers}, T.~C.},
    title = "{A Search for Stars of Very Low Metal Abundance. V. Photoelectric UBV Photometry of Metal-weak Candidates from the Northern HK Survey}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0006178},
 keywords = {Stars: Abundances, Stars: Population II, Techniques: Photometric, Techniques: Spectroscopic},
     year = 2000,
    month = oct,
   volume = 120,
    pages = {2065-2081},
      doi = {10.1086/301566},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....120.2065B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{McCall04,
   author = {{McCall}, M.~L.},
    title = "{On Determining Extinction from Reddening}",
  journal = {\aj},
 keywords = {Stars: Variables: Cepheids, ISM: Dust, Extinction, Galaxies: General, Stars: General, Stars: Supernovae: General, Techniques: Photometric},
     year = 2004,
    month = nov,
   volume = 128,
    pages = {2144-2169},
      doi = {10.1086/424933},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....128.2144M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Harris96,
   author = {{Harris}, W.~E.},
    title = "{A Catalog of Parameters for Globular Clusters in the Milky Way}",
  journal = {\aj},
 keywords = {GLOBULAR CLUSTERS: GENERAL, CATALOGS},
     year = 1996,
    month = oct,
   volume = 112,
    pages = {1487},
      doi = {10.1086/118116},
   adsurl = {http://adsabs.harvard.edu/abs/1996AJ....112.1487H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Williams13,
   author = {{Williams}, M.~E.~K. and {Steinmetz}, M. and {Binney}, J. and 
	{Siebert}, A. and {Enke}, H. and {Famaey}, B. and {Minchev}, I. and 
	{de Jong}, R. and {Boeche}, C. and {Freeman}, K.~C. and {Bienayme}, O. and 
	{Bland-Hawthorn}, J. and {Gibson}, B.~K. and {Gilmore}, G.~F. and 
	{Helmi}, A. and {Kordopatis}, G. and {Munari}, U. and {Navarro}, J.~F. and 
	{Parker}, Q.~A. and {Reid}, W. and {Seabroke}, G.~M. and {Sharma}, S. and 
	{Siviero}, A. and {Watson}, F.~G. and {Wyse}, R.~F.~G. and {Zwitter}, T.
	},
    title = "{The wobbly Galaxy: kinematics north and south with RAVE red clump giants}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1302.2468},
 primaryClass = "astro-ph.GA",
 keywords = {Astrophysics - Galaxy Astrophysics},
     year = 2013,
    month = feb,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1302.2468W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ruchti11,
   author = {{Ruchti}, G.~R. and {Fulbright}, J.~P. and {Wyse}, R.~F.~G. and 
	{Gilmore}, G.~F. and {Bienaym{\'e}}, O. and {Bland-Hawthorn}, J. and 
	{Gibson}, B.~K. and {Grebel}, E.~K. and {Helmi}, A. and {Munari}, U. and 
	{Navarro}, J.~F. and {Parker}, Q.~A. and {Reid}, W. and {Seabroke}, G.~M. and 
	{Siebert}, A. and {Siviero}, A. and {Steinmetz}, M. and {Watson}, F.~G. and 
	{Williams}, M. and {Zwitter}, T.},
    title = "{Observational Properties of the Metal-poor Thick Disk of the Milky Way and Insights into its Origins}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1105.3691},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: disk, stars: abundances, stars: late-type},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {9},
    pages = {9},
      doi = {10.1088/0004-637X/737/1/9},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737....9R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Kordopatis13,
   author = {{Kordopatis}, G. and {Hill}, V. and {Irwin}, M. and {Gilmore}, G. and 
	{Wyse}, R.~F.~G. and {Tolstoy}, E. and {de Laverny}, P. and 
	{Recio-Blanco}, A. and {Battaglia}, G. and {Starkenburg}, E.
	},
    title = "{Through thick and thin: Structure of the Galactic thick disc from extragalactic surveys}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1305.6145},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: evolution, Galaxy: structure, Galaxy: disk, stars: abundances, methods: observational, Galaxy: stellar content},
     year = 2013,
    month = jul,
   volume = 555,
      eid = {A12},
    pages = {A12},
      doi = {10.1051/0004-6361/201321470},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...555A..12K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Demarque04,
   author = {{Demarque}, P. and {Woo}, J.-H. and {Kim}, Y.-C. and {Yi}, S.~K.
	},
    title = "{Y$^{2}$ Isochrones with an Improved Core Overshoot Treatment}",
  journal = {\apjs},
 keywords = {Convection, Stars: Evolution, Stars: Interiors},
     year = 2004,
    month = dec,
   volume = 155,
    pages = {667-674},
      doi = {10.1086/424966},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJS..155..667D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lejeune98,
   author = {{Lejeune}, T. and {Cuisinier}, F. and {Buser}, R.},
    title = "{A standard stellar library for evolutionary synthesis. II. The M dwarf extension}",
  journal = {\aaps},
   eprint = {arXiv:astro-ph/9710350},
 keywords = {STARS: FUNDAMENTAL PARAMETERS, STARS: LATE TYPE},
     year = 1998,
    month = may,
   volume = 130,
    pages = {65-75},
      doi = {10.1051/aas:1998405},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26AS..130...65L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carpenter01,
   author = {{Carpenter}, J.~M.},
    title = "{Color Transformations for the 2MASS Second Incremental Data Release}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0101463},
 keywords = {Infrared Radiation, Standards},
     year = 2001,
    month = may,
   volume = 121,
    pages = {2851-2871},
      doi = {10.1086/320383},
   adsurl = {http://adsabs.harvard.edu/abs/2001AJ....121.2851C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schonrich10,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J. and {Dehnen}, W.},
    title = "{Local kinematics and the local standard of rest}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.3693},
 primaryClass = "astro-ph.GA",
 keywords = {stars: kinematics, Galaxy: disc, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, solar neighbourhood},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {1829-1833},
      doi = {10.1111/j.1365-2966.2010.16253.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403.1829S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gilmore12,
   author = {{Gilmore}, G. and {Randich}, S. and {Asplund}, M. and {Binney}, J. and 
	{Bonifacio}, P. and {Drew}, J. and {Feltzing}, S. and {Ferguson}, A. and 
	{Jeffries}, R. and {Micela}, G. and {Negueruela}, I. and {Prusti}, T. and 
	{Rix}, H.-W. and {Vallenari}, A. and {Alfaro}, E. and {Allende-Prieto}, C. and 
	{Babusiaux}, C. and {Bensby}, T. and {Blomme}, R. and {Bragaglia}, A. and 
	{Flaccomio}, E. and {Fran{\c c}ois}, P. and {Irwin}, M. and 
	{Koposov}, S. and {Korn}, A. and {Lanzafame}, A. and {Pancino}, E. and 
	{Paunzen}, E. and {Recio-Blanco}, A. and {Sacco}, G. and {Smiljanic}, R. and 
	{Van Eck}, S. and {Walton}, N.},
    title = "{The Gaia-ESO Public Spectroscopic Survey}",
  journal = {The Messenger},
     year = 2012,
    month = mar,
   volume = 147,
    pages = {25-31},
   adsurl = {http://adsabs.harvard.edu/abs/2012Msngr.147...25G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Burnett10,
   author = {{Burnett}, B. and {Binney}, J.},
    title = "{Stellar distances from spectroscopic observations: a new technique}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.4367},
 primaryClass = "astro-ph.IM",
 keywords = {methods: numerical, methods: statistical, techniques: photometric, techniques: spectroscopic, astrometry, stars: distances},
     year = 2010,
    month = sep,
   volume = 407,
    pages = {339-354},
      doi = {10.1111/j.1365-2966.2010.16896.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407..339B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{Kordopatis11a,
   author = {{Kordopatis}, G. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Bijaoui}, A. and {Hill}, V. and {Gilmore}, G. and {Wyse}, R.~F.~G. and 
	{Ordenovic}, C.},
    title = "{Automatic stellar spectra parameterisation in the IR Ca ii triplet region}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.6237},
 primaryClass = "astro-ph.IM",
 keywords = {stars: fundamental parameters, stars: abundances, techniques: spectroscopic, methods: data analysis},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A106},
    pages = {A106},
      doi = {10.1051/0004-6361/201117372},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A.106K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kordopatis11b,
   author = {{Kordopatis}, G. and {Recio-Blanco}, A. and {de Laverny}, P. and 
	{Gilmore}, G. and {Hill}, V. and {Wyse}, R.~F.~G. and {Helmi}, A. and 
	{Bijaoui}, A. and {Zoccali}, M. and {Bienaym{\'e}}, O.},
    title = "{A spectroscopic survey of thick disc stars outside the solar neighbourhood}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.5221},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: evolution, Galaxy: kinematics and dynamics, stars: abundances, methods: observational},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A107},
    pages = {A107},
      doi = {10.1051/0004-6361/201117373},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A.107K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gazzano13,
   author = {{Gazzano}, J.-C. and {Kordopatis}, G. and {Deleuil}, M. and 
	{de Laverny}, P. and {Recio-Blanco}, A. and {Hill}, V.},
    title = "{Characterisation of the Galactic thin disc with CoRoT targets}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1301.0111},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: stellar content, Galaxy: disk, Galaxy: structure, Galaxy: evolution, Galaxy: kinematics and dynamics},
     year = 2013,
    month = feb,
   volume = 550,
      eid = {A125},
    pages = {A125},
      doi = {10.1051/0004-6361/201117747},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...550A.125G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Schlegel98,
   author = {{Schlegel}, D.~J. and {Finkbeiner}, D.~P. and {Davis}, M.},
    title = "{Maps of Dust Infrared Emission for Use in Estimation of Reddening and Cosmic Microwave Background Radiation Foregrounds}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9710327},
 keywords = {COSMOLOGY: DIFFUSE RADIATION, COSMOLOGY: COSMIC MICROWAVE BACKGROUND, ISM: DUST, EXTINCTION, INTERPLANETARY MEDIUM, INFRARED: ISM: CONTINUUM},
     year = 1998,
    month = jun,
   volume = 500,
    pages = {525},
      doi = {10.1086/305772},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...500..525S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{NissenSchuster2010,
   author = {{Nissen}, P.~E. and {Schuster}, W.~J.},
    title = "{Two distinct halo populations in the solar neighborhood. Evidence from stellar abundance ratios and kinematics}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1002.4514},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, stars: kinematics and dynamics, Galaxy: halo, Galaxy: formation},
     year = 2010,
    month = feb,
   volume = 511,
      eid = {L10},
    pages = {L10},
      doi = {10.1051/0004-6361/200913877},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...511L..10N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ishigaki,
   author = {{Ishigaki}, M.~N. and {Aoki}, W. and {Chiba}, M.},
    title = "{Chemical Abundances of the Milky Way Thick Disk and Stellar Halo. II. Sodium, Iron-peak, and Neutron-capture Elements}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1306.0954},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: formation, Galaxy: halo, stars: abundances},
     year = 2013,
    month = jul,
   volume = 771,
      eid = {67},
    pages = {67},
      doi = {10.1088/0004-637X/771/1/67},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...771...67I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schonrich2009,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J.},
    title = "{Origin and structure of the Galactic disc(s)}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0907.1899},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc , solar neighbourhood , galaxies: abundances , galaxies: evolution , galaxies: ISM , galaxies: kinematics and dynamics},
     year = 2009,
    month = nov,
   volume = 399,
    pages = {1145-1156},
      doi = {10.1111/j.1365-2966.2009.15365.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009MNRAS.399.1145S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shonrich09NoThick,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J.},
    title = "{Chemical evolution with radial mixing}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0809.3006},
 keywords = {galaxies: abundances , galaxies: evolution , galaxies: ISM , galaxies: kinematics and dynamics , Galaxy: disc , solar neighbourhood},
     year = 2009,
    month = jun,
   volume = 396,
    pages = {203-222},
      doi = {10.1111/j.1365-2966.2009.14750.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.396..203S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Spagna2010,
   author = {{Spagna}, A. and {Lattanzi}, M.~G. and {Re Fiorentin}, P. and 
	{Smart}, R.~L.},
    title = "{Evidence of a thick disk rotation-metallicity correlation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1002.0074},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, Galaxy: kinematics and dynamics, Sun:, abundances, stars: kinematics and dynamics, surveys},
     year = 2010,
    month = feb,
   volume = 510,
      eid = {L4},
    pages = {L4},
      doi = {10.1051/0004-6361/200913538},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...510L...4S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Minchev12,
   author = {{Minchev}, I. and {Chiappini}, C. and {Martig}, M.},
    title = "{The Chemodynamical Evolution of the Milky Way Disc I: The Solar Vicinity}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1208.1506},
 primaryClass = "astro-ph.GA",
 keywords = {Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2012,
    month = aug,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012arXiv1208.1506M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Minchev13,
   author = {{Minchev}, I. and {Chiappini}, C. and {Martig}, M. and {Steinmetz}, M. and 
	{de Jong}, R.~S. and {Boeche}, C. and {Scannapieco}, C. and 
	{Zwitter}, T. and {Wyse}, R.~F.~G. and {Binney}, J.~J. and {Bland-Hawthorn}, J. and 
	{Bienayme}, O. and {Famaey}, B. and {Gibson}, B.~K. and {Grebel}, E.~K. and 
	{Gilmore}, G. and {Helmi}, A. and {Kordopatis}, G. and {Lee}, Y.~S. and 
	{Munari}, U. and {Navarro}, J.~F. and {Parker}, Q.~A. and {Quillen}, A.~C. and 
	{Reid}, W.~A. and {Siebert}, A. and {Siviero}, A. and {Seabroke}, G. and 
	{Watson}, F. and {Williams}, M.},
    title = "{A new stellar chemo-kinematic relation reveals the merger history of the Milky Way disc}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1310.5145},
 primaryClass = "astro-ph.GA",
 keywords = {Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
     year = 2013,
    month = oct,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013arXiv1310.5145M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Misiroitis,
   author = {{Misiriotis}, A. and {Xilouris}, E.~M. and {Papamastorakis}, J. and 
	{Boumis}, P. and {Goudis}, C.~D.},
    title = "{The distribution of the ISM in the Milky Way. A three-dimensional large-scale model}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0607638},
 keywords = {dust, extinction, ISM: structure, Galaxy: structure},
     year = 2006,
    month = nov,
   volume = 459,
    pages = {113-123},
      doi = {10.1051/0004-6361:20054618},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006A%26A...459..113M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Morrison,
   author = {{Morrison}, H.~L. and {Flynn}, C. and {Freeman}, K.~C.},
    title = "{Where does the disk stop and the halo begin? Kinematics in a rotation field}",
  journal = {\aj},
 keywords = {G STARS, GALACTIC ROTATION, GIANT STARS, K STARS, MILKY WAY GALAXY, STELLAR MOTIONS, ABUNDANCE, ANGULAR VELOCITY, STATISTICAL ANALYSIS, VELOCITY DISTRIBUTION},
     year = 1990,
    month = oct,
   volume = 100,
    pages = {1191-1222},
      doi = {10.1086/115587},
   adsurl = {http://adsabs.harvard.edu/abs/1990AJ....100.1191M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carollo,
   author = {{Carollo}, D. and {Beers}, T.~C. and {Chiba}, M. and {Norris}, J.~E. and 
	{Freeman}, K.~C. and {Lee}, Y.~S. and {Ivezi{\'c}}, {\v Z}. and 
	{Rockosi}, C.~M. and {Yanny}, B.},
    title = "{Structure and Kinematics of the Stellar Halos and Thick Disks of the Milky Way Based on Calibration Stars from Sloan Digital Sky Survey DR7}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0909.3019},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, Galaxy: formation, Galaxy: halo, Galaxy: kinematics and dynamics, methods: data analysis, stars: abundances},
     year = 2010,
    month = mar,
   volume = 712,
    pages = {692-727},
      doi = {10.1088/0004-637X/712/1/692},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010ApJ...712..692C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sofue,
   author = {{Sofue}, Y. and {Honma}, M. and {Omodaka}, T.},
    title = "{Unified Rotation Curve of the Galaxy -- Decomposition into de Vaucouleurs Bulge, Disk, Dark Halo, and the 9-kpc Rotation Dip --}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {0811.0859},
 keywords = {Galaxy: bulge, Galaxy: disk, Galaxy: rotation curve, Galaxy: structure},
     year = 2009,
    month = feb,
   volume = 61,
    pages = {227-},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009PASJ...61..227S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Demers,
   author = {{Demers}, S. and {Battinelli}, P.},
    title = "{C stars as kinematic probes of the Milky Way disk from 9 to 15 kpc}",
  journal = {\aap},
 keywords = {stars: carbon, stars: kinematics, Galaxy: disk, Galaxy: kinematics and dynamics},
     year = 2007,
    month = oct,
   volume = 473,
    pages = {143-148},
      doi = {10.1051/0004-6361:20077691},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...473..143D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{MishaGrad,
   author = {{Haywood}, M.},
    title = "{Radial mixing and the transition between the thick and thin Galactic discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0805.1822},
 keywords = {Galaxy: abundances , Galaxy: evolution , solar neighbourhood},
     year = 2008,
    month = aug,
   volume = 388,
    pages = {1175-1184},
      doi = {10.1111/j.1365-2966.2008.13395.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.388.1175H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pedicelli,
   author = {{Pedicelli}, S. and {Bono}, G. and {Lemasle}, B. and {Fran{\c c}ois}, P. and 
	{Groenewegen}, M. and {Lub}, J. and {Pel}, J.~W. and {Laney}, D. and 
	{Piersimoni}, A. and {Romaniello}, M. and {Buonanno}, R. and 
	{Caputo}, F. and {Cassisi}, S. and {Castelli}, F. and {Leurini}, S. and 
	{Pietrinferni}, A. and {Primas}, F. and {Pritchard}, J.},
    title = "{On the metallicity gradient of the Galactic disk}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0906.3140},
 primaryClass = "astro-ph.SR",
 keywords = {stars: variables: Cepheids, galaxy: disk, stars: oscillations, stars: abundances, stars: evolution , galaxy: stellar content},
     year = 2009,
    month = sep,
   volume = 504,
    pages = {81-86},
      doi = {10.1051/0004-6361/200912504},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...504...81P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Rudolph,
   author = {{Rudolph}, A.~L. and {Fich}, M. and {Bell}, G.~R. and {Norsen}, T. and 
	{Simpson}, J.~P. and {Haas}, M.~R. and {Erickson}, E.~F.},
    title = "{Abundance Gradients in the Galaxy}",
  journal = {\apjs},
 keywords = {Galaxy: Abundances, ISM: H II Regions, ISM: Abundances},
     year = 2006,
    month = feb,
   volume = 162,
    pages = {346-374},
      doi = {10.1086/498869},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJS..162..346R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Andreuzzi,
   author = {{Andreuzzi}, G. and {Bragaglia}, A. and {Tosi}, M. and {Marconi}, G.
	},
    title = "{Old open clusters and the Galactic metallicity gradient: Berkeley 20, Berkeley 66 and Tombaugh 2}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1011.2349},
 primaryClass = "astro-ph.GA",
 keywords = {Hertzsprung-Russell and colour-magnitude diagrams, Galaxy: disc, open clusters and associations: general, open clusters and associations: individual: Berkeley 20, open clusters and associations: individual: Berkeley 66, open clusters and associations: individual: Tombaugh 2},
     year = 2011,
    month = apr,
   volume = 412,
    pages = {1265-1282},
      doi = {10.1111/j.1365-2966.2010.17986.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011MNRAS.412.1265A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magrini,
   author = {{Magrini}, L. and {Sestito}, P. and {Randich}, S. and {Galli}, D.
	},
    title = "{The evolution of the Galactic metallicity gradient from high-resolution spectroscopy of open clusters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0812.0854},
 keywords = {Galaxy: disk, Galaxy: abundances, Galaxy: evolution, open clusters and associations: general},
     year = 2009,
    month = jan,
   volume = 494,
    pages = {95-108},
      doi = {10.1051/0004-6361:200810634},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009A%26A...494...95M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magrini10,
   author = {{Magrini}, L. and {Randich}, S. and {Zoccali}, M. and {Jilkova}, L. and 
	{Carraro}, G. and {Galli}, D. and {Maiorca}, E. and {Busso}, M.
	},
    title = "{Open clusters towards the Galactic centre: chemistry and dynamics. A VLT spectroscopic study of NGC 6192, NGC 6404, NGC 6583}",
  journal = {\aap},
 keywords = {Galaxy: abundances, Galaxy: evolution, open clusters and associations: individual: NGC 6192, open clusters and associations: individual: NGC 6404, open clusters and associations: individual: NGC 6583},
     year = 2010,
    month = nov,
   volume = 523,
      eid = {A11},
    pages = {A11},
      doi = {10.1051/0004-6361/201015395},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...523A..11M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Boeche,
   author = {{Boeche}, C. and {Chiappini}, C. and {Minchev}, I. and {Williams}, M. and 
	{Steinmetz}, M. and {Sharma}, S. and {Kordopatis}, G. and {Bland-Hawthorn}, J. and 
	{Bienaym{\'e}}, O. and {Gibson}, B.~K. and {Gilmore}, G. and 
	{Grebel}, E.~K. and {Helmi}, A. and {Munari}, U. and {Navarro}, J.~F. and 
	{Parker}, Q.~A. and {Reid}, W. and {Seabroke}, G.~M. and {Siebert}, A. and 
	{Siviero}, A. and {Watson}, F.~G. and {Wyse}, R.~F.~G. and {Zwitter}, T.
	},
    title = "{The relation between chemical abundances and kinematics of the Galactic disc with RAVE}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1302.3466},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: evolution, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2013,
    month = may,
   volume = 553,
      eid = {A19},
    pages = {A19},
      doi = {10.1051/0004-6361/201219607},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26A...553A..19B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ivezic,
   author = {{Ivezi{\'c}}, {\v Z}. and {Sesar}, B. and {Juri{\'c}}, M. and 
	{Bond}, N. and {Dalcanton}, J. and {Rockosi}, C.~M. and {Yanny}, B. and 
	{Newberg}, H.~J. and {Beers}, T.~C. and {Allende Prieto}, C. and 
	{Wilhelm}, R. and {Lee}, Y.~S. and {Sivarani}, T. and {Norris}, J.~E. and 
	{Bailer-Jones}, C.~A.~L. and {Re Fiorentin}, P. and {Schlegel}, D. and 
	{Uomoto}, A. and {Lupton}, R.~H. and {Knapp}, G.~R. and {Gunn}, J.~E. and 
	{Covey}, K.~R. and {Smith}, J.~A. and {Miknaitis}, G. and {Doi}, M. and 
	{Tanaka}, M. and {Fukugita}, M. and {Kent}, S. and {Finkbeiner}, D. and 
	{Munn}, J.~A. and {Pier}, J.~R. and {Quinn}, T. and {Hawley}, S. and 
	{Anderson}, S. and {Kiuchi}, F. and {Chen}, A. and {Bushong}, J. and 
	{Sohi}, H. and {Haggard}, D. and {Kimball}, A. and {Barentine}, J. and 
	{Brewington}, H. and {Harvanek}, M. and {Kleinman}, S. and {Krzesinski}, J. and 
	{Long}, D. and {Nitta}, A. and {Snedden}, S. and {Lee}, B. and 
	{Harris}, H. and {Brinkmann}, J. and {Schneider}, D.~P. and 
	{York}, D.~G.},
    title = "{The Milky Way Tomography with SDSS. II. Stellar Metallicity}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0804.3850},
 keywords = {Galaxy: Halo, Galaxy: Kinematics and Dynamics, Galaxy: Stellar Content, Galaxy: Structure, Methods: Data Analysis, Stars: Statistics},
     year = 2008,
    month = sep,
   volume = 684,
    pages = {287-325},
      doi = {10.1086/589678},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...684..287I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haywood2006,
   author = {{Haywood}, M.},
    title = "{Revisiting two local constraints of the Galactic chemical evolution}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0609523},
 keywords = {Galaxy: abundances: Galaxy: evolution: solar neighbourhood, Galaxy: abundances, Galaxy: evolution, solar neighbourhood},
     year = 2006,
    month = oct,
   volume = 371,
    pages = {1760-1776},
      doi = {10.1111/j.1365-2966.2006.10802.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006MNRAS.371.1760H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yong05,
   author = {{Yong}, D. and {Carney}, B.~W. and {Teixera de Almeida}, M.~L.
	},
    title = "{Elemental Abundance Ratios in Stars of the Outer Galactic Disk. I. Open Clusters}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0504193},
 keywords = {Galaxy: Abundances, Galaxy: Disk, Galaxy: Open Clusters and Associations: General},
     year = 2005,
    month = aug,
   volume = 130,
    pages = {597-625},
      doi = {10.1086/430934},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005AJ....130..597Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Carney,
   author = {{Carney}, B.~W. and {Yong}, D. and {Teixera de Almeida}, M.~L. and 
	{Seitzer}, P.},
    title = "{Elemental Abundance Ratios in Stars of the Outer Galactic Disk. II. Field Red Giants}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0506210},
 keywords = {Galaxy: Abundances, Galaxy: Disk},
     year = 2005,
    month = sep,
   volume = 130,
    pages = {1111-1126},
      doi = {10.1086/432541},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005AJ....130.1111C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yong06,
   author = {{Yong}, D. and {Carney}, B.~W. and {Teixera de Almeida}, M.~L. and 
	{Pohl}, B.~L.},
    title = "{Elemental Abundance Ratios in Stars of the Outer Galactic Disk. III. Cepheids}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0512348},
 keywords = {Galaxy: Abundances, Galaxy: Disk},
     year = 2006,
    month = apr,
   volume = 131,
    pages = {2256-2273},
      doi = {10.1086/500538},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006AJ....131.2256Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Binney,
   author = {{Binney}, J.},
    title = "{More dynamical models of our Galaxy}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1207.4917},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, solar neighbourhood, galaxies: kinematics and dynamics},
     year = 2012,
    month = oct,
   volume = 426,
    pages = {1328-1337},
      doi = {10.1111/j.1365-2966.2012.21692.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.426.1328B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burnett,
   author = {{Burnett}, B.},
  journal = {DPhil thesis, Oxford University},
archivePrefix = "arXiv",
     year = 2010,
}

@ARTICLE{LuckLambert11,
   author = {{Luck}, R.~E. and {Lambert}, D.~L.},
    title = "{The Distribution of the Elements in the Galactic Disk. III. A Reconsideration of Cepheids from l = 30{\deg} to 250{\deg}}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1108.1947},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: evolution, stars: abundances, stars: variables: Cepheids},
     year = 2011,
    month = oct,
   volume = 142,
      eid = {136},
    pages = {136},
      doi = {10.1088/0004-6256/142/4/136},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011AJ....142..136L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Lemasle13,
   author = {{Lemasle}, B. and {Francois}, P. and {Genovali}, K. and {Kovtyukh}, V.~V. and 
	{Bono}, G. and {Inno}, L. and {Laney}, C.~D. and {Kaper}, L. and 
	{Bergemann}, M. and {Fabrizio}, M. and {Matsunaga}, N. and {Pedicelli}, S. and 
	{Primas}, F. and {Romaniello}, M.},
    title = "{Galactic abundance gradients from Cepheids: alpha and heavy elements in the outer disk}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1308.3249},
 primaryClass = "astro-ph.GA",
 keywords = {Astrophysics - Galaxy Astrophysics},
     year = 2013,
    month = aug,
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013arXiv1308.3249L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{BovyApogee,
   author = {{Bovy}, J. and {Allende Prieto}, C. and {Beers}, T.~C. and {Bizyaev}, D. and 
	{da Costa}, L.~N. and {Cunha}, K. and {Ebelke}, G.~L. and {Eisenstein}, D.~J. and 
	{Frinchaboy}, P.~M. and {Garc{\'{\i}}a P{\'e}rez}, A.~E. and 
	{Girardi}, L. and {Hearty}, F.~R. and {Hogg}, D.~W. and {Holtzman}, J. and 
	{Maia}, M.~A.~G. and {Majewski}, S.~R. and {Malanushenko}, E. and 
	{Malanushenko}, V. and {M{\'e}sz{\'a}ros}, S. and {Nidever}, D.~L. and 
	{O'Connell}, R.~W. and {O'Donnell}, C. and {Oravetz}, A. and 
	{Pan}, K. and {Rocha-Pinto}, H.~J. and {Schiavon}, R.~P. and 
	{Schneider}, D.~P. and {Schultheis}, M. and {Skrutskie}, M. and 
	{Smith}, V.~V. and {Weinberg}, D.~H. and {Wilson}, J.~C. and 
	{Zasowski}, G.},
    title = "{The Milky Way's Circular-velocity Curve between 4 and 14 kpc from APOGEE data}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1209.0759},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, Galaxy: fundamental parameters, Galaxy: general, Galaxy: kinematics and dynamics, Galaxy: structure, stars: kinematics and dynamics},
     year = 2012,
    month = nov,
   volume = 759,
      eid = {131},
    pages = {131},
      doi = {10.1088/0004-637X/759/2/131},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...759..131B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miyamoto,
   author = {{Miyamoto}, M. and {Nagai}, R.},
    title = "{Three-dimensional models for the distribution of mass in galaxies}",
  journal = {\pasj},
 keywords = {ASTRONOMICAL MODELS, DENSITY DISTRIBUTION, GALACTIC STRUCTURE, MASS DISTRIBUTION, POTENTIAL THEORY, THREE DIMENSIONAL MODELS, FUNCTIONS (MATHEMATICS), GLOBULAR CLUSTERS, GRAVITATIONAL EFFECTS, MATHEMATICAL MODELS, MILKY WAY GALAXY},
     year = 1975,
   volume = 27,
    pages = {533-543},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1975PASJ...27..533M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hernquist,
   author = {{Hernquist}, L.},
    title = "{An analytical model for spherical galaxies and bulges}",
  journal = {\apj},
 keywords = {COMPUTATIONAL ASTROPHYSICS, ELLIPTICAL GALAXIES, GALACTIC BULGE, GALACTIC STRUCTURE, ASTRONOMICAL MODELS, ASTRONOMICAL PHOTOMETRY, BRIGHTNESS DISTRIBUTION, DISTRIBUTION FUNCTIONS},
     year = 1990,
    month = jun,
   volume = 356,
    pages = {359-364},
      doi = {10.1086/168845},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1990ApJ...356..359H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cheng12,
   author = {{Cheng}, J.~Y. and {Rockosi}, C.~M. and {Morrison}, H.~L. and 
	{Lee}, Y.~S. and {Beers}, T.~C. and {Bizyaev}, D. and {Harding}, P. and 
	{Malanushenko}, E. and {Malanushenko}, V. and {Oravetz}, D. and 
	{Pan}, K. and {Schlesinger}, K.~J. and {Schneider}, D.~P. and 
	{Simmons}, A. and {Weaver}, B.~A.},
    title = "{A Short Scale Length for the {$\alpha$}-enhanced Thick Disk of the Milky Way: Evidence from Low-latitude SEGUE Data}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1204.5179},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: abundances, Galaxy: disk, Galaxy: evolution, Galaxy: formation},
     year = 2012,
    month = jun,
   volume = 752,
      eid = {51},
    pages = {51},
      doi = {10.1088/0004-637X/752/1/51},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...752...51C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Sales09,
   author = {{Sales}, L.~V. and {Helmi}, A. and {Abadi}, M.~G. and {Brook}, C.~B. and 
	{G{\'o}mez}, F.~A. and {Ro{\v s}kar}, R. and {Debattista}, V.~P. and 
	{House}, E. and {Steinmetz}, M. and {Villalobos}, {\'A}.},
    title = "{Orbital eccentricity as a probe of thick disc formation scenarios}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0909.3858},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc , Galaxies: kinematics and dynamics , galaxies: formation},
     year = 2009,
    month = nov,
   volume = 400,
    pages = {L61-L65},
      doi = {10.1111/j.1745-3933.2009.00763.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009MNRAS.400L..61S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilson11,
   author = {{Wilson}, M.~L. and {Helmi}, A. and {Morrison}, H.~L. and {Breddels}, M.~A. and 
	{Bienaym{\'e}}, O. and {Binney}, J. and {Bland-Hawthorn}, J. and 
	{Campbell}, R. and {Freeman}, K.~C. and {Fulbright}, J.~P. and 
	{Gibson}, B.~K. and {Gilmore}, G. and {Grebel}, E.~K. and {Munari}, U. and 
	{Navarro}, J.~F. and {Parker}, Q.~A. and {Reid}, W. and {Seabroke}, G. and 
	{Siebert}, A. and {Siviero}, A. and {Steinmetz}, M. and {Williams}, M.~E.~K. and 
	{Wyse}, R.~F.~G. and {Zwitter}, T.},
    title = "{Testing formation mechanisms of the Milky Way's thick disc with RAVE}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1009.2052},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disc, Galaxy: formation, solar neighbourhood, Galaxy: structure},
     year = 2011,
    month = may,
   volume = 413,
    pages = {2235-2241},
      doi = {10.1111/j.1365-2966.2011.18298.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011MNRAS.413.2235W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mishenina13,
   author = {{Mishenina}, T.~V. and {Pignatari}, M. and {Korotin}, S.~A. and 
	{Soubiran}, C. and {Charbonnel}, C. and {Thielemann}, F.-K. and 
	{Gorbaneva}, T.~I. and {Basak}, N.~Y.},
    title = "{Abundances of neutron-capture elements in stars of the Galactic disk substructures}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1303.1730},
 primaryClass = "astro-ph.SR",
 keywords = {nuclear reactions, nucleosynthesis, abundances, stars: abundances, stars: late-type, Galaxy: evolution},
     year = 2013,
    month = apr,
   volume = 552,
      eid = {A128},
    pages = {A128},
      doi = {10.1051/0004-6361/201220687},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26A...552A.128M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fraternali13,
   author = {{Fraternali}, F. and {Marasco}, A. and {Marinacci}, F. and {Binney}, J.
	},
    title = "{Ionized Absorbers as Evidence for Supernova-driven Cooling of the Lower Galactic Corona}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1301.4998},
 primaryClass = "astro-ph.GA",
 keywords = {galaxies: evolution, galaxies: ISM, galaxies: star formation, Galaxy: halo, ISM: clouds},
     year = 2013,
    month = feb,
   volume = 764,
      eid = {L21},
    pages = {L21},
      doi = {10.1088/2041-8205/764/2/L21},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013ApJ...764L..21F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Adibekyan2011,
   author = {{Adibekyan}, V.~Z. and {Santos}, N.~C. and {Sousa}, S.~G. and 
	{Israelian}, G.},
    title = "{A new {$\alpha$}-enhanced super-solar metallicity population}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.4936},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, stars: kinematics and dynamics, Galaxy: disk},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {L11},
    pages = {L11},
      doi = {10.1051/0004-6361/201118240},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...535L..11A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fuhrmann11,
   author = {{Fuhrmann}, K.},
    title = "{Nearby stars of the Galactic disc and halo - V}",
  journal = {\mnras},
 keywords = {stars: fundamental parameters, Galaxy: evolution, Galaxy: formation, Galaxy: stellar content},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {2893-2922},
      doi = {10.1111/j.1365-2966.2011.18476.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011MNRAS.414.2893F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reddy06,
   author = {{Reddy}, B.~E. and {Lambert}, D.~L. and {Allende Prieto}, C.
	},
    title = "{Elemental abundance survey of the Galactic thick disc}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0512505},
 keywords = {stars: abundances, stars: kinematics, Galaxy: abundances, Galaxy: evolution},
     year = 2006,
    month = apr,
   volume = 367,
    pages = {1329-1366},
      doi = {10.1111/j.1365-2966.2006.10148.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006MNRAS.367.1329R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fuhrmann04,
   author = {{Fuhrmann}, K.},
    title = "{Nearby stars of the Galactic disk and halo. III.}",
  journal = {Astronomische Nachrichten},
 keywords = {stars: fundamental parameters, Galaxy: formation, Galaxy: stellar content, Galaxy: evolution},
     year = 2004,
    month = jan,
   volume = 325,
    pages = {3-80},
      doi = {10.1002/asna.200310173},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2004AN....325....3F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gustafsson08,
   author = {{Gustafsson}, B. and {Edvardsson}, B. and {Eriksson}, K. and 
	{J{\o}rgensen}, U.~G. and {Nordlund}, {\AA}. and {Plez}, B.},
    title = "{A grid of MARCS model atmospheres for late-type stars. I. Methods and general properties}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0805.0554},
 keywords = {stars: atmospheres, Sun: abundances, stars: fundamental parameters, stars: general, stars: late-type, stars: supergiants},
     year = 2008,
    month = aug,
   volume = 486,
    pages = {951-970},
      doi = {10.1051/0004-6361:200809724},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008A%26A...486..951G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grevesse07,
   author = {{Grevesse}, N. and {Asplund}, M. and {Sauval}, A.~J.},
    title = "{The Solar Chemical Composition}",
  journal = {\ssr},
 keywords = {Sun: abundances, photosphere, corona},
     year = 2007,
    month = jun,
   volume = 130,
    pages = {105-114},
      doi = {10.1007/s11214-007-9173-7},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007SSRv..130..105G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nissen11,
   author = {{Nissen}, P.~E. and {Schuster}, W.~J.},
    title = "{Two distinct halo populations in the solar neighborhood. II. Evidence from stellar abundances of Mn, Cu, Zn, Y, and Ba}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1103.4755},
 primaryClass = "astro-ph.GA",
 keywords = {stars: atmospheres, stars: abundances, Galaxy: abundances, Galaxy: halo, Galaxy: formation},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A15},
    pages = {A15},
      doi = {10.1051/0004-6361/201116619},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...530A..15N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schuster12,
   author = {{Schuster}, W.~J. and {Moreno}, E. and {Nissen}, P.~E. and {Pichardo}, B.
	},
    title = "{Two distinct halo populations in the solar neighborhood. III. Evidence from stellar ages and orbital parameters}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1111.4026},
 primaryClass = "astro-ph.GA",
 keywords = {stars: abundances, Galaxy: halo, stars: kinematics and dynamics, Galaxy: evolution},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A21},
    pages = {A21},
      doi = {10.1051/0004-6361/201118035},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...538A..21S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sellwood02,
   author = {{Sellwood}, J.~A. and {Binney}, J.~J.},
    title = "{Radial mixing in galactic discs}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0203510},
 keywords = {ISM: abundances, Galaxy: abundances, Galaxy: kinematics and dynamics, galaxies: evolution, galaxies: ISM, galaxies: structure},
     year = 2002,
    month = nov,
   volume = 336,
    pages = {785-796},
      doi = {10.1046/j.1365-8711.2002.05806.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002MNRAS.336..785S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Roskar08,
   author = {{Ro{\v s}kar}, R. and {Debattista}, V.~P. and {Quinn}, T.~R. and 
	{Stinson}, G.~S. and {Wadsley}, J.},
    title = "{Riding the Spiral Waves: Implications of Stellar Migration for the Properties of Galactic Disks}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {0808.0206},
 keywords = {Galaxies: Evolution, Galaxies: Spiral, Galaxies: Stellar Content, Galaxy: Stellar Content, Galaxy: Solar Neighborhood, Stellar Dynamics},
     year = 2008,
    month = sep,
   volume = 684,
    pages = {L79-L82},
      doi = {10.1086/592231},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...684L..79R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schonrich2009b,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J.},
    title = "{Chemical evolution with radial mixing}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0809.3006},
 keywords = {galaxies: abundances , galaxies: evolution , galaxies: ISM , galaxies: kinematics and dynamics , Galaxy: disc , solar neighbourhood},
     year = 2009,
    month = jun,
   volume = 396,
    pages = {203-222},
      doi = {10.1111/j.1365-2966.2009.14750.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2009MNRAS.396..203S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fuhrmann98,
   author = {{Fuhrmann}, K.},
    title = "{Nearby stars of the Galactic disk and halo}",
  journal = {\aap},
 keywords = {STARS: DISTANCES, STARS: FUNDAMENTAL PARAMETERS, STARS: LATE-TYPE, GALAXY: EVOLUTION},
     year = 1998,
    month = oct,
   volume = 338,
    pages = {161-183},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1998A%26A...338..161F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Edvardsson93,
   author = {{Edvardsson}, B. and {Andersen}, J. and {Gustafsson}, B. and 
	{Lambert}, D.~L. and {Nissen}, P.~E. and {Tomkin}, J.},
    title = "{The Chemical Evolution of the Galactic Disk - Part One - Analysis and Results}",
  journal = {\aap},
     year = 1993,
    month = aug,
   volume = 275,
    pages = {101},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1993A%26A...275..101E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ricardo11,
   author = {{Carrera}, R. and {Pancino}, E.},
    title = "{Chemical abundance analysis of the open clusters Berkeley 32, NGC 752, Hyades, and Praesepe}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1107.2242},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, open clusters and associations: individual: NGC 752, open clusters and associations: individual: Hyades, open clusters and associations: individual: Berkeley 32, open clusters and associations: individual: Preasepe (M 44), stars: abundances},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201117473},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...535A..30C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Katz11,
   author = {{Katz}, D. and {Soubiran}, C. and {Cayrel}, R. and {Barbuy}, B. and 
	{Friel}, E. and {Bienaym{\'e}}, O. and {Perrin}, M.-N.},
    title = "{Probing the Galactic thick disc vertical properties and interfaces}",
  journal = {\aap},
 keywords = {Galaxy: disk, stars: abundances, Galaxy: abundances},
     year = 2011,
    month = jan,
   volume = 525,
      eid = {A90},
    pages = {A90},
      doi = {10.1051/0004-6361/201014840},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011A%26A...525A..90K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Burkert92,
   author = {{Burkert}, A. and {Truran}, J.~W. and {Hensler}, G.},
    title = "{The collapse of our Galaxy and the formation of the Galactic disk}",
  journal = {\apj},
 keywords = {COSMOCHEMISTRY, DWARF STARS, GALACTIC EVOLUTION, GRAVITATIONAL COLLAPSE, MILKY WAY GALAXY, GLOBULAR CLUSTERS, KINEMATICS, METALLICITY, STAR FORMATION},
     year = 1992,
    month = jun,
   volume = 391,
    pages = {651-658},
      doi = {10.1086/171378},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1992ApJ...391..651B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{LeeAlphas,
   author = {{Lee}, Y.~S. and {Beers}, T.~C. and {An}, D. and {Ivezi{\'c}}, {\v Z}. and 
	{Just}, A. and {Rockosi}, C.~M. and {Morrison}, H.~L. and {Johnson}, J.~A. and 
	{Sch{\"o}nrich}, R. and {Bird}, J. and {Yanny}, B. and {Harding}, P. and 
	{Rocha-Pinto}, H.~J.},
    title = "{Formation and Evolution of the Disk System of the Milky Way: [{$\alpha$}/Fe] Ratios and Kinematics of the SEGUE G-dwarf Sample}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1104.3114},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: disk, Galaxy: formation, Galaxy: kinematics and dynamics, Galaxy: structure},
     year = 2011,
    month = sep,
   volume = 738,
      eid = {187},
    pages = {187},
      doi = {10.1088/0004-637X/738/2/187},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2011ApJ...738..187L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{WyseLag,
   author = {{Wyse}, R.~F.~G. and {Gilmore}, G. and {Norris}, J.~E. and {Wilkinson}, M.~I. and 
	{Kleyna}, J.~T. and {Koch}, A. and {Evans}, N.~W. and {Grebel}, E.~K.
	},
    title = "{Further Evidence of a Merger Origin for the Thick Disk: Galactic Stars along Lines of Sight to Dwarf Spheroidal Galaxies}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0601308},
 keywords = {Galaxy: Evolution, Galaxy: Kinematics and Dynamics, Galaxy: Stellar Content, Galaxy: Structure},
     year = 2006,
    month = mar,
   volume = 639,
    pages = {L13-L16},
      doi = {10.1086/501228},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006ApJ...639L..13W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{BensbyFeltzing10,
   author = {{Bensby}, T. and {Feltzing}, S.},
    title = "{The Galactic thin and thick disks in the context of galaxy formation}",
 keywords = {stars: abundances, stars: kinematics, Galaxy: abundances, Galaxy: disk},
booktitle = {IAU Symposium},
     year = 2010,
   series = {IAU Symposium},
   volume = 265,
archivePrefix = "arXiv",
   eprint = {0908.3807},
 primaryClass = "astro-ph.GA",
   editor = {{Cunha}, K. and {Spite}, M. and {Barbuy}, B.},
    month = mar,
    pages = {300-303},
      doi = {10.1017/S1743921310000773},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010IAUS..265..300B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


